The Belle II Detector Upgrades Framework Conceptual Design Report

We describe the planned near-term and potential longer-term upgrades of the Belle II detector at the SuperKEKB electron-positron collider operating at the KEK laboratory in Tsukuba, Japan. These upgrades will allow increasingly sensitive searches for possible new physics beyond the Standard Model in flavor, tau, electroweak and dark sector physics that are both complementary to and competitive with the LHC and other experiments.

==> 04.PhysicsPerformance/Physics.tex <==
\section{Physics case with 50 ab$^{-1}$ and detector challenges}

The physics case of the \belletwo\ Experiment, which is extensively covered in~\cite{Belle-II:2018jsg} and \cite{Belle-II:2022cgf}, includes a large number of precision measurements on observables of $B$- and $D$-meson and $\tau$-lepton decays that are sensitive to fundamental parameters of the standard model and could be sensitive to the existence of particles and couplings not envisioned by the theory. A significant part of the physics programme consists of searches of exotic multiquark states that challenge the traditional QCD models and of fundamentally new particles that are connected to a Dark Sector extension of the standard model.

In order to achieve those goals, it is fundamental that the \belletwo\ detector maintains its performance, in terms of reconstruction efficiencies and
resolutions of the various physics objects, close to the design levels. During the first years of operations, the experiment has observed higher than anticipated levels of machine-related backgrounds, and a consequent degradation of the physics performance. Mitigating these backgrounds through revised machine design and beam tuning and counteracting their effects with targeted detector upgrades will be crucial to attain our physics goals.

In this section we will compare the different upgrade scenarios in terms of their performance on some selected physics channels, chosen based on their importance within the physics programme or on their specific sensitivity to the experimental aspects.

In section~\ref{sec:perf_strategy} we will outline the strategy for evaluating and comparing the physics reach of the different upgrade scenarios, that will be based on analyzing Monte Carlo simulated samples reconstructed with different detector configurations and under either optimistic or conservative background scenarios. In the following sections we will review the results on the physics channels, grouped based on their sensitivity to tracking (sec.~\ref{sec:perf_tracking}), particle identification (\ref{sec:perf_pid}), neutrals (\ref{sec:perf_neutrals}), and trigger (\ref{sec:perf_neutrals}).


\section{Performance evaluation strategy}
\label{sec:perf_strategy}

The choice of the upgrade scenarios will be based on considerations of feasibility, cost, and effectiveness in terms of physics reach. In order to evaluate the latter, we generate samples of Monte Carlo simulated data for a number of physics channels of interest and use them to evaluate specific quantities (efficiency, resolution, discrimination power, ... ) that characterize the performance of the detector. 

We generate samples of adequate size utilizing the current Belle II detector configuration and the proposed upgrade scenarios and for each we consider different machine background assumptions.

In order to speed up the process and produce minimal impact to the ongoing activities, the evaluation of the performance is carried out by analyzing the simulated samples described above with the same strategy and analysis code that is currently being used in actual Belle II physics analyses. The exercise could also provide positive feedback to the analysts and suggest ways to improve the Belle II physics reach.


\section{Tracking}
\label{sec:perf_tracking}

\subsection{Tracking efficiency}

Tracking efficiency plays an important role for the vast majority of physics channels that are of interest in Belle II.

One of the key features of the $B$-factories is the possibility of reconstructing the decay of one of the two $B$ mesons in the event into fully hadronic final states or semileptonic decays in which only the neutrino(s) are unreconstructed \cite{Keck:2018lcd}. This allows analysts to assign all the remaining particles in the event to the decay of the remaining $B$ in the event, thus achieving a much better control on the backgrounds.

Notable examples of channels that utilize this technique are $B^+ \to \tau^+ \nu$ and $B \to D^{(*)} \tau \nu$, which are characterized by at least one neutrino in the final state, and therefor difficult to separate kinematically from the main backgrounds without taking the full event into consideration. Given the need to reconstruct a relatively large number of charged particles, the sensitivity on these channels strongly depends on the tracking (in)efficiency.

Another important channel for Belle II is $B+ \to D^0 K^+$, with $D^0 \to K^0_S \pi^+ \pi^-$, which is sensitive to the CKM angle $\phi_3 / \gamma$ and has five charged particles in the final state, two of which significantly displaced from the interaction region.


\subsection{Low momentum tracking efficiency}

Another advantage of Belle II consists in the ability to reconstruct charged particles with low transverse momentum (in the range $50 < p_T < 200$ MeV/$c$), which is particularly important for reconstructing $D^{*+} \to D^0 \pi^+$ decays, which occur in a variety of analyses. Due to the limited phase space, the momentum of the pion is typically below 200 MeV/$c$ at Belle II, and thus it is often referred to as a "soft" or "slow" pion.

Also in this section we utilize the $B \to D^{(*)} \tau \nu$ decays to measure the low momentum tracking efficiency.


\subsection{Reconstruction of long lived particles}

The reconstruction of particles that fly a considerable distance (a few cm or more) from their production vertex is a requirement in many areas of the Belle II physics program. In this section we focus on $K^0_S$'s or particles that behave similarly and decay to a pair of charged particles within the tracking volume of the detector.

We utilize the channels $B^0 \to K^0_S \pi^0$ and \textcolor{red}{add a DS channel with long lived particles} to evaluate the reconstruction efficiency for long lived particles.


\subsection{Vertexing resolution}

Time dependent analyses are a key part of the beauty and charm program of Belle II. The sensitivity to fundamental parameters of the standard model depends on our ability to determine the position of decay vertices. 

The golden channel for this section is $B^0 \to J/\psi K^0_S$. In Table~\ref{tab:vertexing_resolution}, we compare the resolutions on the positions of the signal-side and tag-side $B$-decay vertices, and on the proper decay time difference $\Delta t$, which is the main observable for time dependent $CP$ violation analyses.

%% example table

\begin{landscape}
\begin{table}[htbp]
\centering

\begin{tabular}{l|ccc|ccc|ccc}
\hline\hline
$B^0 \to J/\psi K^0_S$ & \multicolumn{3}{c|}{Belle II} & \multicolumn{3}{c|}{VTX} & \multicolumn{3}{c}{other} \\
 & BGx1 & BGx2 & BGx5 & BGx1 & BGx2 & BGx5 & BGx1 & BGx2 & BGx5 \\
\hline
$B_{sig}$ vertex resolution [$\mu$m] &     
  x.x & y.y & z.z & x.x & y.y & z.z & x.x & y.y & z.z \\
$B_{tag}$ vertex resolution [$\mu$m] &   
  x.x & y.y & z.z & x.x & y.y & z.z & x.x & y.y & z.z \\
$\Delta t$ resolution [ps] &   
  x.x & y.y & z.z & x.x & y.y & z.z & x.x & y.y & z.z \\
\hline\hline

\end{tabular}
\caption{Example table.}
\label{tab:vertexing_resolution}

\end{table}
\end{landscape}




\section{Particle identification (PID)}
\label{sec:perf_pid}

In this section we concentrate on the $K/\pi$ separation capability of the detector. At low momentum (below $\sim 1$ GeV/$c$), we mostly rely on the specific energy loss $dE/dx$ which is provided by the tracking detectors, while at higher momenta, the contribution of the dedicated PID devices becomes more important.

\subsection{dE/dx resolution}

We compare the $K/\pi$ separation capabilities of the different detector configurations at low momentum by considering the $B^{+/0} \to K^+K^-K^{+/0}$ final state, for which often two charged kaons originate from the decay of a $\phi$ resonance, and typically have relatively low momentum.

\subsection{Performance of the dedicated PID devices}

To evaluate the PID performance at high $K/\pi$ momenta, we study the $B \to K \pi$ and $B \to (K^*/\rho) \, \gamma$ channels, for which the particle momenta approach the kinematic limit of the decay products of $B$ mesons. Especially in the latter case, characterized by relatively broad and overlapping resonances, particle identification is a fundamental tool to enhance/suppress the $b \to s$ component over the $b \to d$. 


\section{Neutrals}
\label{sec:perf_neutrals}

Final states containing neutral particles are particularly important at Belle II, as it can exploit the advantages of the relatively clean and kinematically constrained environment of the $e^+e^-$ collisions. In the following subsections we will compare the performance of the detector scenarios under study for photons, neutral pions, and neutral kaons.

\subsection{Photon reconstruction efficiency and energy resolution}

The reconstruction efficiency and resolution in the measurement of the energy of photons is key for the separating an elusive signal from the backgrounds.

We concentrate on the $D^0 \to \gamma \gamma$ and $\tau \to \mu \gamma$ decays, which are very suppressed or forbidden in the standard model, and are among those for which Belle II will have a unique sensitivity.

On the other hand, the ability to correctly identify photons and precisely measure their energy is instrumental for the analyses that heavily rely on the measurement of the \textit{extra energy} in the event, that is the energy that is not associated to any of the final state particles of the decay considered. The $B^+ \to \tau^+ \nu$ and $B \to D^{(*)} \tau \nu$ are two examples of such analyses.

\subsection{$\pi^0$ reconstruction efficiency and mass resolution}

For the impact on the $\pi^0$ reconstruction efficiency and resolution, we consider the channels $B^0 \to \pi^0\pi^0$ and $B^0 \to K^0_S \pi^0$, that critically depend on $\pi^0$ performance for the neutrals reconstruction, and also $B^0 \to \eta^{\prime} K^0$, for which the decay chain $\eta^{\prime} \to \eta \pi^+\pi^-$, $\eta \to \pi^+\pi^-\pi^0$ is an important contribution.

\subsection{$K^0_L$ reconstruction efficiency}

We evaluate the performance on $K^0_L$ reconstruction using the golden channel $B^0 \to J/\psi K^0_L$. 

$K^0_L$ reconstruction plays also a role on inclusive $V_{ub}$ analyses, as $K^0$'s typically originate from a $b \to c$ cascade, and thus their presence is a valuable handle to suppress the backgrounds coming from the more frequent $B \to D^{(*, **)} \ell \nu$ decays.

\section{Trigger}
\label{sec:perf_trigger}

\subsection{Low multiplicity final states}
\subsection{High multiplicity final states}


\section{Summary}







==> 05.InnerDetector/S2.MAPS-old.tex <==
\section{CMOS MAPS}
\label{sec:MAPS}
%\editor{C.Marinas, J.Baudot}

The VTX proposal consists in exploiting demonstrated performance of current CMOS monolithic active pixel sensor (MAPS) to replace the VXD system with 5 detection layers uniformly equipped with the same fast, light and granular sensor. The VTX solution reduces by at least two orders of magnitude the current PXD integration time and replaces the double-sided strip sensors of the SVD by real 2D-pixel detectors, with the following expected benefits:
\begin{itemize}
\item Ability to cope with larger background levels than the current VXD, thanks to a low detector occupancy alleviating any data transmission bottleneck and
allowing a resilient track finding efficiency with respect to hit-rate.
\item Improved momentum resolution and impact parameter resolution at low transverse momentum, performance being robust against scaled backgrounds. In general, the tracking chain is simplified with all layers involved in the track finding algorithm, allowing also for natural tracking alternatives (inside-out tracking).
\item Simplified and lighter services due to smaller cross sections of the data cables and less complex cooling system. The detector integration is expected to be simple allowing an installation over one long summer shutdown. Fewer material in front of the endcaps gives additional room for extra shielding in the interaction region and bellows to protect the outer detectors. Current machine-detector interface boundaries can be kept or slightly changed if required by modifications of the final focusing system. 
\item Direct connection to the standard Belle II data acquisition path due to the low transmission bandwidth and input source to the high level and level 1 triggers. Completely standalone 5-layer tracker available for pattern recognition.
\item Operation are simplified since no special mode of operation (e.g. Gated Mode) nor data reduction (e.g. ROI selection) are required. Due to the usage of the same sensor all over, the control and power system becomes unique.
\end{itemize}
Though all layers use the same sensor, their designs differ due to their active length varying from 12 to 70 cm to cover the required acceptance. While the two innermost layers follow an all-silicon ladder concept (iVTX), the outermost (oVTX) layers require carbon fiber support structures and flex print cables.
The VTX targets an overall material budget in the range 1.5-2.0\%~$X_0$ and will be the first light and compact MAPS-based vertex-tracker operating at an high-rate $e^+e^-$ collider.  

\begin{figure}[htb]
\begin{center}
\includegraphics*[width=12cm]{figures/vtx5-3dmodel.png}
\caption{Overall VTX layout.}
\end{center}
\label{figure:VTX}
\end{figure}


\subsection{Technological solutions}

The CMOS sensor for the VTX project relies on the CIS-180 nm process by Tower Semiconductor 
(https://towersemi.com/technology/cmos\_image\_sensor/). Intense R\&D has been carried out with this process since about ten years in the high-energy physics community and lead to major successes \cite{aglieri_rinella_alpide_2017,bespin_dmaps_2020,deveaux_observations_2019}. Especially the depleted MAPS TJ-MONOPIX-2 \cite{moustakas_design_2021} offer essential features already matching the requirements for Belle II VXD sensors.
\begin{itemize}
\item The sensitive volume is made of an epitaxial layer with thickness between 18 and 40~$\mu$m and a
high resistivity (in excess of 1 k$\Omega$.cm) for a sizeable signal generation and an additional shallow
layer (so-called modified process) to ensure full depletion, which is critical for radiation
tolerance.
\item Four wells and six metal layers are available, allowing for a design of complex circuitry within the
pixel and over the matrix, thus facilitating the implementation of advanced read-out
architectures needed to cope with the high data rate expected.
\item The maximal dimensions of the process reticle implemented on 8” wafers reaches $25\times 31$~cm$^2$ matching well the expected size for the VTX sensor of about $20\times 30$~cm$^2$.
\item The thinning of MAPS is actually one of their key benefits. The possibility to thin sensors down to about
60 or 50~$\mu$m has been demonstrated in various projects and for vast quantities of chips over the past 10
years.
\end{itemize}
The sensor dedicated to the Belle II VTX is called OBELIX and its main design features are summarised in table \ref{table:OBELIX}. \\

\begin{center}
\begin{table}[htb]
\caption{Design features of the OBELIX sensor.}
\centering
\begin{tabular}{ | l | r | } 
\hline
Pixel pitch & 30 to 40 $\mu$m \\
\hline
Matrix size & 512 rows $\times$ 928 to 752 columns \\
\hline
Time stamping & 25 to 100 ns precision over 7 bits \\
\hline
Signal Time over threshold & 7 bits \\
\hline
Output bandwidth & 320 to 640 Mbps \\ 
\hline
Power dissipation & 100 to 200 mW/cm$^2$ \\
\hline
Radiation tolerance & 100 MRad and $10^{14}$ n$_{\mathrm{eq}}$/cm$^2$\\
\hline
\end{tabular}
\label{table:OBELIX}
\end{table}
\end{center}

The two innermost layers, namely iVTX, targets an individual material budget of about $0.1$\%~$X_0$. Such light layer is possible due to the moderate overall surface of these layers, below 400~cm$^2$, the low sensor power dissipation and the few connections needed for the sensor operations. First such conditions makes air cooling a viable solution. Then in addition, the all-silicon ladder is essentially made of four contiguous OBELIX sensors diced out of production wafers thinned to 50~$\mu$m except in some areas still featuring few hundreds of $\mu$m thickness to insure mechanical stability. A post-processing step etches additional metal strips to interconnect sensors along the ladder and provides a unique connector at the ladder end.\\
   
\begin{figure}[htb]
\begin{center}
\includegraphics*[width=12cm]{figures/iVTX-ladder-concept.png}
\caption{Schematic view of the iVTX ladder design.}
\end{center}
\label{figure:iVTX}
\end{figure}

A more traditional approach drives the oVTX ladder concept for outer layers, strongly inspired by the design successfully developed for the ALICE ITS2 \cite{fantoni_upgrade_2020}. Each ladder is made of a light carbon fiber support structure, a cold plate including tubes for water leakless circulation, two rows of sensors glued on the cold plate and finally two flex print cables connecting each half the sensors to a single end-ladder connector. Depending on their radius, the material budget of individual oVTX ladders ranges from 0.3 to 0.5\%~$X_0$. \\

\begin{figure}[htb]
\begin{center}
\includegraphics*[width=12cm]{figures/oVTX-ladder-concept.png}
\caption{Schematic view of the oVTX ladder design.}
\end{center}
\label{figure:oVTX}
\end{figure}


The proposed VTX detector is expected to be operated at room temperature. The low sensor occupancy leads to moderate data rates to be extracted. These aspects result in a dramatic reduction of services with respect to the current VXD. Consequently, similar or simpler overall mechanical support, cabling and acquisition system are required and are not further described here. In particular, the standard PCIe40 \cite{daq:pcie40} acquisition boards used in Belle~II match well the data throughput requirement.


\subsection{Design work and schedule}

Assuming a potential installation for the new VTX subsystem in 2026, the coarse project schedule is to develop all technical solutions till early 2023, then produce all parts and assemble them to have a complete detector in early 2026. Additional 10 to 12 months will be needed to ship all parts to KEK and perform the required re-assembly and tests before inserting the complete instrument into the Belle II system. Though the deadline for the development phase might appear ambitious, it has to be noted that numerous solutions are already pre-existing as described below.\\

The OBELIX sensor is based on the pixel matrix of the TJ-MONOPIX-2 chip, which is itself an optimised successor of an earlier version TJ-MONOPIX-1 \cite{bespin_dmaps_2020}. 
 The design of the first CMOS MAPS dedicated to Belle~II, OBELIX-1, has started in 2021 and targets a fabrication mid-2022, allowing for the full characterisation by 2023. The main design work to complete OBELIX-1 consists in extending the TJ-MONOPIX-2 pixel matrix, adding power regulators for easier power distribution system and of course develop an end-of-column digital adapted to the Belle~II triggering scheme. In addition, simulation and test studies on the front-end used in TJ-MONOPIX-2 shall indicate how much power can be spared if the integration time is enlarged. Currently, the front-end allows hit-tagging at 25~ns, while physics simulations demonstrated that 100~ns ({\it reference to section where simulation performance described}) is sufficient with respect to the expected hit rate. Operating the front-end at a lower current and/or lower frequency will lower the power dissipation toward 100~mW/cm$^2$ compared to the expected current baseline of 200~mW/cm$^2$.\\
 
 The iVTX full-silicon concept is currently being assessed with industrial partners, first using dummy silicon wafers and in the near future with real sensors. Key parts of the oVTX ladder, the longest carbon fiber support structure and flex cable have been prototyped and fabricated. Their tests shall allow a validation of the full ladder design. For both concepts initial proof of concept results are expected in 2022.
 
\subsection{The VTX collaboration}

The VTX proposal encompasses the main critical hardware aspects of the development required for a vertex detector: sensors, detection layers, acquisition system. The work is currently conducted by a still open collaboration of seventeen groups from five countries: Austria (HEPHY-Vienna), France (CPPM-Marseille, IJCLab-Orsay, IPHC-Strasbourg), Germany (UNiversity of Bonn, University of Dortmund, University of Goettingen, KIT-Karlsruhe), Italy (University of Bergamo, INFN-Pavia, INFN \& University of Pisa), Spain (IFAE-Barcelona, IMB-CNM-CSIC-Barcelona, IFCA-CSIC-UC-Santander, IMSE-CNM-CSIC-Seville, IFIC-CSIC-UV-Valencia, ITAINNOVA-Zaragoza).

\subsection{Cost estimation}

Based on the experience from other projects exploiting the CMOS-MAPS technology, especially the recent ALICE ITS2 \cite{fantoni_upgrade_2020}, an initial rough cost for the VTX was established. This estimation assume a VTX with five detection layers, corresponding to 16 iVTX ladders, 64 oVTX ladders and about 2200 CMOS sensors. Table \ref{tab:VTXcost} breaks down the various component costs (without the beam pipe) including the development and production phases.

\begin{center}
\begin{table}[htb]
\caption{Initial cost estimation in k\$ for the VTX project}
\centering
\begin{tabular}{ | l | r | r | r | } \hline
{\bf Component} & {\bf Development } & {\bf Production} & {\bf Total (k\$)} \\ 
\hline
 CMOS sensors & 600 & 900 & 1,500 \\ 
 Ladders & 200 & 600 & 800 \\
 Assembly & 100 & 500 & 600 \\
 Mechanics & 50 & 150 & 200 \\
 DAQ \& Services & 300 & 1,000 & 1,300 \\
\hline
 {\bf Total } & 1,250 & 3,150 & {\bf 4,400} \\ 
\hline
\end{tabular}
\label{tab:VTXcost}
\end{table}
\end{center}


==> 06.OuterDetector/S1.TOP.tex <==
\section{TOP}
\label{sec:TOP}
\editor{E.Torassa}

\subsection{Introduction}

With four years of running experience at Belle II, the world-record luminosity of SuperKEKB has been accompanied by higher than anticipated backgrounds.  
%Fig. 1
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.55]{fig/TOP/TOPmodule.pdf}
\caption{\it Illustration of the back side of one TOP module where electronic boards and photodetectors are interfaced with the quartz prism and quartz bar.}
\label{fig:TOPmodule}
\end{center}
\end{figure}
For the TOP subsystem (Fig.~\ref{fig:TOPmodule}) this implies that the hit rate and the quantum efficiency degradation of the Micro-Channel Plate Photomultiplier Tubes (MCP-PMTs) must be monitored to assess the risk that even the last generation, the life-extended atomic layer deposition ALD MCP-PMTs, may not survive until the target integrated luminosity. 

R\&D has started on a possible silicon photomultiplier (SiPM) replacement option. This option looks promising, although the required cooling will reduce the space available for the readout electronics and limit its acceptable heat load. Thermal gradients and potential thermal and mechanical stresses need to be carefully evaluated. 

Moreover, the projected high rates of Single Event Upsets (SEUs) is problematic, as some number of them are not recoverable and will lead to increasing data taking loss.  There are concerns about the radiation tolerance of the fiber optic transceiver modules connecting the front-end to the back-end electronic boards. Simulations indicated a fairly low radiation of 10 Gy/year with a corresponding expected lifetime of 20 years larger than intrinsic lifetime, but the real background can be largely underestimated. 
%Fig. 2
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.55]{fig/TOP/TOP-PMT-QE.pdf}
\caption{Expected QE degradation for the three different generations of MCP-PMTs installed in the TOP detector: conventional, ALD and life-extended ALD.  Horizontal axis shows the year and vertical axis is the relative QE.}
\label{fig:QEprojection}
\end{center}
\end{figure}

The timescale for replacement of the TOP photosensors is related to the level of background during the next years.  
Fig.~\ref{fig:QEprojection} shows a projection of the expected PMT quantum-efficiency (QE) degradation.
The Monte Carlo expected background was considered for the components related to the luminosity (Bhabha scattering, two-photon processes) and a maximum limit of 5 MHz/PMT for the other components (beam-gas, Touschek). The expected gradual increase in peak luminosity described in~\cite{top:topupgrade} was taken into account. In this case, the QE of normal ALD type PMTs will drop below 80~\% starting from 2027 and all PMTs will reach this level of QE degradation at around the current luminosity target.
Some MCP-PMTs showed a faster than expected reduction in QE considering their accumulated charge. One possible explanation is that they operated at a higher temperature for some time due to a temporary 
overheating of the electronics. 
Quantum-efficiency measurements performed in the laboratory as a function of the accumulated charge show a faster degradation at higher temperatures (Fig.~\ref{fig:MCP-PMTheat}).  
New readout electronics with reduced power consumption can help to increase the MCP-PMT's lifetime.
% Fig. 3
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.62]{fig/TOP/MCP-PMTheat.pdf}
\caption{Relative QE degradation as a function of the accumulated charge at $20\degrees C$ and $40\degrees C$ for two conventional MCP-PMTs.}
\label{fig:MCP-PMTheat}
\end{center}
\end{figure}
%

Planning has started for these upgrades, which could take place during a  long shutdown to rebuild the interaction region on the timescale of roughly 5 years from now. 

\subsection{TOP program summary}

The rudimentary schedule and cost estimates for the electronic readout are based upon production and delivery of the 8k channels of TOP readout.  This endeavor leverages heavily two sizeable past and new investments: re-use of existing infrastructure and firmware, wherever possible and development of ASICs appropriate to the TOP upgrade.
In both cases the pre-production plus production timescale is approximately 2 years, with 6-9 months for installation and commissioning.  Based upon the preliminary prototyping being performed and costed separately from this, the total project cost is estimated to be 3.1 M$\$$ for upgrades to the TOP readout systems.
For the photosensors the primary option is the replacement of normal ALD PMTs with life extended ALD MCP-PMTs once the installed PMTs approach the end of their lifetime.
With this option, we need ~220 new MCP-PMTs to replace normal ALD type PMTs, at an estimated costs of 1.6 M$\$$. The production of life-extended ALD MCP-PMT has already restarted, 90 MCP-PMTs have been ordered, 30 of them have been delivered. A further improvement in the ALD technology
and the MCP-PMTs replacement with cold SiPMs are the possible solutions if the increase of luminosity leads to a rapid loss of efficiency of the life extended ALD MCP-PMTs.

\subsection{Upgrade proposal}

The goals of the baseline upgrade to the readout electronics are twofold: reduce significantly their size, as well as the power required.  Both goals facilitate the implementation of the requisite cooling needed to operate the SiPMs in single-photon detection (though with significantly increased dark-count) mode.

In order to reduce cost and development time, much of the existing software, firmware and hardware infrastructure can be retained.  The boundary conditions considered for this costing exercise are:

\begin{itemize}
    \item retain the Standard Control Read-Out Data (SCROD) board, the existing cables, low-voltage power system and the existing infrastructure for the TOP-based online event time logic of the L1 trigger in TOP FEE;
    \item remove the HV divider chain/delivery board and associated cables;
    \item employ multiple Analog to digital converter System-on-Chip (ASoC) developed by Nalu Scientific.
%    per ASIC "Carrier" card, each with multiple Gbps connections to the SCROD FPGA
\end{itemize}

 Nalu Scientific, LLC (NSL) is a small business in Honolulu, HI and was originally a spin-off of the University of Hawaii’s High Energy Physics group back in 2016.  NSL works closely with US DOE laboratories and universities. It has developed commercially available variations of the IRSX and TARGETX chips that had been used for TOP and KLM readout.  Further development and refinement of the IRSX and TARGETX ASICs has led to a new generation of chips: the ASoC (Analog to digital converter System on a Chip)~\cite{top:ASoC} and the HDSoC (High Density digitizer System on a Chip)~\cite{top:HDSoC3}. The ASoC and HDSoC include on chip circuitry and functionality to perform sampling, digitization, triggering, region of interest extraction operations. Essentially, an analog channel enters the chip and packetized data exits the chip in high speed serial form. The chips operate with a high level of autonomy, which reduces the need for high-end FPGAs on the readout board. The ASoCv3 is a 4 channel digitizer with 16k samples of buffer per channel operating at 2.5-4 GSa/s channel. It is commercially available with a suite of test hardware, firmware, software and documentation. Version 3 (a four-channel chip) has been tested and has improved power consumption compared to the IRSX. It can be used for bench testing and development purposes starting immediately.
A custom version of the ASoC (ASoCv4) is proposed for the TOP readout upgrade with 8 channels per chip, which is matched to the existing readout infrastructure and has improved speed and power consumption. This new ASIC (ASoCv4) would be developed for the TOP upgrade. 
The ASoC can communicate with less complex FPGAs (compared to IRSX) which will reduce size, cost, power consumption, and SEU issues while maintaining overall firmware backwards compatibility with the current IRSX based system. 
%Based upon this proposed modification, the upgraded readout system still consists of 64 "board stacks" and 4 ASIC "carrier" cards per "board stack".  The new ASIC "carrier" card will no longer have a FPGA to reduce radiation fault events and employ eight 4-channel readout AISCs per card with point-to-point Gbit serial links to the SCROD FPGA. 

For the photosensors, the Hamamatsu production line of life-extended ALD MCP-PMT is still operating with an expected output of 10 MCP-PMTs/month. A possible further increase of lifetime can be investigated for example by an optimization of the atomic layer thickness.

The option of MCP-PMT replacement requires several studies and possibly further SiPM developments with the goal to reduce the dark count rate.
It is important to find the best balance among different SiPM's characteristics:
single device size, single cell dimension, operating temperature.
Considering the expected neutron rate near the photodetector region at the target instantaneous luminosity of $6\times 10^{35}cm^{-2}s^{-1}$ is about \SI{2.0 e 10}{n/(cm^2 \cdot~year)}, we need to be able to distinguish single photons at least up to an irradiation of  \SI{1 e 11}{n/cm^2}, even more for higher luminosity. We need also to retain photon efficiency, a good time resolution and have acceptable thermal and mechanical stresses for the detector.
The single channel active area of the MCP-PMT with 16 channels and $1~in^2$ size is about $6 \times 6~mm^2$. Smaller SiPMs have been considered to limit the impact of the dark count rate to the single photoelectron spectrum. 
Sixteen Hamamtsu SiPMs  $1.3 \times 1.3~mm^2$ size and 50 $\mu m$ cells have been irradiated from \SI{1.03 e 09}{n/cm^2} to \SI{5.07 e 11}{n/cm^2}. 
%Fig. 4
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.60]{fig/TOP/SinglePhotonSpectrum.pdf}
\caption{Single photoelectron spectrum (number of entries vs signal amplitude in ADC counts) for an irradiation of \SI{5.07 e 11}{n/cm^2} (left) and  \SI{5.07 e 10}{n/cm^2} (right) at different temperatures. Signal peaks have been fitted with the convolution of a Poisson distribution with some double Gaussian functions (dashed lines), a Gaussian background (yellow) has been added to the fit.}
\label{fig:SinglePhoton}
\end{center}
\end{figure}
%
The single photon spectra are shown in Fig.~\ref{fig:SinglePhoton} for two different irradiations at different temperatures. In the most critical condition with \SI{5.07 e 11}{n/cm^2} and 20 \textdegree C the single photon peak cannot be distinguished from the dark count background.
From this preliminary test SiPMs operating at -20 \textdegree C is a possible solution also with a factor of 5 safety margin. However it should be noted that using  $1.3 \times 1.3~mm^2$ SiPMs will require  ~20 times more electronic channels 
or a multiplexing downstream of the SiPM amplification.

The expected improvements in the SuperKEK instantaneous luminosity will require to tighten the readout timing windows in most detector subsystems. As the result, the TOP-based contribution to the online event time logic of the L1 trigger will become even more important. Significant backgrounds expected in the future call for novel machine learning and artificial intelligence algorithms to be implemented in the trigger firmware logic of the existing trigger boards UT4. We anticipate also to take full advantage of the new trigger board UT5 which is based on Versal FPGA architecture and is being developed at KEK. This work will also require to upgrade firmware of the trigger path in TOP FEE. Backend TOPTRG L1 work is further discussed in the TRG section of this CDR. 

\subsection{Design development and human resources}

The design of the electronics for the readout of all the channels digitized by the new ASoCv4 is still to be defined. To properly estimate the power consumption reduction full details of the new boards are needed.

The primary option for the photosensors is to replace the older ALD MCP-PMTs, when they reach their lifetime limit, with life-extended ALD MCP-PMTs. 

It is anticipated that  Nagoya U., INFN/U. Padova and INFN/U. Torino will work on the photosensor upgrade, while Indiana U, U. Hawaii, U. Pittsburgh and Nalu Scientific personnel will contribute to the electronics upgrade.

The TOP-based L1 trigger work in TOP FEE and in the TOP TRG system will be performed by U. Hawaii and U. Pittsburgh with (being discussed) contributions from other universities and laboratories.

\subsection{Cost and schedule}

It is anticipated that 1.5 FTE of engineering effort is required for the design of the carrier card board in years 1 and 2. In addition 1 postdoc and 1 graduate student will assist with assembly, test and documentation under the oversight of the U. Hawaii instrumentation frontier professor.
Board fabrication and assembly costs are based upon those realized during earlier prototyping. After the pre-production a yearly firmware development engineering support is costed during the 2 years of production, and at a reduced level during commissioning.
The estimated costs of the electronics upgrade are described in Table~\ref{iTOP:table1}. The estimated costs for the replacement of the 220 ALD MCP-PMTs are described in Table~\ref{iTOP:table2} for the life-extended ALD MCP-PMT option and in Table~\ref{iTOP:table3} for the SiPM option. 
The estimated cost of human resources for TOP-based TOP FEE and L1 trigger work is 0.5 FTE (from base funding). Estimates of the costs associated with the new trigger boards are discussed in the TRG section of this CDR. 
%
\begin{table}[htb]
\caption{TOP readout electronics upgrade cost estimate.}
\centering
\begin{tabularx}{\textwidth}{ | l | l | X | r | } \hline
\multicolumn{4}{|c|}{\bf ASoC ASIC readout Upgrade } \\ \hline
{\bf Phase}    & {\bf Resource}              & {\bf Basis of estimate} & {\bf Cost (k\$)} \\ \hline
Pre-production & Engineering \& test         & 1.5 FTE       & 610 \\ 
               & Parts procur. \& assembly   & cost summary  & 120 \\ \hline
Production     & Engineering \& test         & 1.5 FTE       & 610 \\ 
               & Parts procur. \& assembly   & cost summary  & 800 \\ \hline
System test    & Beam test         & past experience with IRSX   & 500 \\ \hline 
Commissioning  & Integration \& Installation & 1.0 FTE       & 445 \\ \hline
Subtotal       &     \multicolumn{2}{|r|}{}                  & 3085 \\ \hline
Contingency (20 \%) & \multicolumn{2}{|r|}{}                  & 617 \\ \hline
{\bf Total} & \multicolumn{2}{|r|}{}                  & {\bf 3702} \\ \hline
\end{tabularx}
\label{iTOP:table1}
\end{table}
%
\begin{table}[htb]
\caption{Life-extended ALD MCP-PMT upgrade cost estimate}
\centering
\begin{tabular}{ | l | l | l | r | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Production & MCP-PMT Production & Engr. est. & 1500 \\  
           & MCP-PMT Test & Engr. est. & 15 \\
           & Assembly parts & Engr. est. & 50  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
{\bf Total} & & & {\bf 1615} \\ \hline \hline
\end{tabular}
\label{iTOP:table2}
\end{table}
%
\begin{table}[htb]
\caption{SiPM upgrade cost estimate}
\centering
\begin{tabular}{ | l | l | l | r | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Pre-production & Engineering & 0.5 FTE & 50\\ 
 & SiPM R\&D & Engr. est. &  10 \\ 
 & Cooling R\&D & Engr. est. & 50 \\ \hline
 Production & Engineering & 0.5 FTE & 50 \\  
 & SiPM + assembly parts & Engr. est. & 700 \\
 & Cooling system & Engr. est. & 100  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
 Contingency (20 \%) &  &  & 202 \\  \hline 
 {\bf Total} & & & {\bf 1212} \\ \hline \hline
\end{tabular}
\label{iTOP:table3}
\end{table}


==> 06.OuterDetector/S1.TOP_Gary.tex <==
\section{TOP}
\label{sec:TOP}
\editor{E.Torassa}

\subsection{Introduction}

With three years of running experience at Belle II, the world-record luminosity of SuperKEKB has been accompanied by higher than anticipated backgrounds.  For the TOP subsystem this means it is looking increasingly likely that even the life-extended Atomic Layer Deposition Micro-Channel Plate Photomultiplier Tubes (ALD MCP-PMTs) may not survive until the target integrated luminosity.  R\&D has started on a possible silicon photomultiplier (SiPM) replacement option. This option looks promising, although the required cooling will reduce the space available for the readout electronics and limit its acceptable heat load. Anyway thermal gradients and potential thermal and mechanical stresses need to be carefully evaluated. Moreover, the projected high rates of Single Event Upsets (SEUs) is problematic, as some number of them are not recoverable and will lead to increasing data taking loss.  Perhaps of greater concern is the known/measured lack of radiation tolerance of the fiber optic transceiver modules. The readout electronics upgrade has been considered as well.


The timescale for replacement of the TOP photosensors is related to the level of background during the next years. Fig.~\ref{fig:QEprojection} shows the expected projection of PMT quantum-efficiency (QE) degradation. The Monte Carlo expected background was considered for the components related to the luminosity (Bhabha scattering, two-photon processes) and a maximum limit of 5 MHz/PMT for the other components (beam-gas, Touschek). In this case, the QE of normal ALD type PMTs will become less than 80~\% starting from 2027 and all PMTs will reach this level of QE degradation at around the end of the current luminosity target.

Planning has started for these upgrades happening during a possible long shutdown to rebuild the interaction region on the timescale of roughly 5 years from now. 

%Fig. 1
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{figures/TOP/TOP-PMT-QE.pdf}
\caption{\it Expected projection of QE degradation for the three different generations of MCP-PMTs installed in the TOP detector: conventional, ALD and life-extended ALD.  Horizontal axis shows the year and vertical axis is the relative QE.}
\label{fig:QEprojection}
\end{center}
\end{figure}

\subsection{Executive Summary}

The rudimentary schedule and cost estimates for the electronic readout are based upon production and delivery of the 8k channels of TOP readout and 20k channels of KLM scintillator readout, as well as the KLM data concentrators.  This endeavor leverages heavily two sizeable past and new investments: re-use of existing infrastructure and firmware, wherever possible; and DOE supported "Small Business Innovation Research" (SBIR) funding for development of ASICs appropriate to these upgrades.  

In both cases the pre-production plus production timescale is approximately 2 years, with 6-9 months for installation and commissioning.  Based upon the preliminary prototyping being performed and costed separately from this, the total project cost is estimated to be 1.1-1.3 M$\$$ and 1.4-1.8 M$\$$ for upgrades to the TOP and KLM readout systems, respectively, depending upon amplifier choices.

For the photosensors the primary option for the upgrade in 2026 is the replacement of normal ALD PMTs with life-extended ALD type PMTs.
With this option, we need ~220 new MCP-PMTs to replace normal
ALD type PMTs, which costs is estimated to be 1.5 M$\$$ and requires to start the mass-production from JFY2021. The production of life-extended ALD MCP-PMT already restarted, 30 MCP-PMT have been ordered and will be delivered within JFY2021. The backup option is the replacement of MCP-PMTs with cold SiPMs. For further luminosity upgrade, SiPMs operated at low temperature is the primary option. 

%\clearpage

\subsection{Upgrade Proposal}

The goals of baseline upgrade to the readout electronics are twofold: reduce significantly their size, as well as the power required.  Both goals facilitate the implementation of the requisite cooling needed to operate the SiPMs in single-photon detection (though with significantly increased dark-count) mode.

In order to reduce cost and development time, much of the existing software, firmware and hardware infrastructure can be retained.  The boundary conditions considered for this costing exercise are:

\begin{itemize}
    \item Retain the Standard Control Read-Out Data (SCROD) board, the existing cables and low-voltage power system
    \item Remove the HV divider chain/delivery board and associated cables
    \item Employ 32-channel TOP System on Chip readout ASICs, each with multiple Gbps connections to the SCROD FPGA
    \item 2 different amplifier options for the Si-PMs are considered and costed
\end{itemize}

%The basic revised architecture is illustrated in Fig.~\ref{fig:TOPupgrade}, where the interface plane to the PMTs is pushed back from the current PoGO pin location and is serviced by a single, new Carrier card containing four 32-channel TOPSoC ASICs, which communicate directly with the retained SCROD Rev B.

%% - Fig 2
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.75]{figs/TOPupgrade.pdf}
%\caption{\it Baseline design for upgrade of the readout "boardstack". A photo at left, and at right schematically
%the proposed replacement.}
%\label{fig:TOPupgrade}
%\end{center}
%\end{figure}
 
Based upon this proposed modification, the upgraded readout system still consists of 64 "board stacks", though there is now a single "Carrier" card containing four 32-channel readout AISCs replacing the current four "Carrier" cards containing four 8-channel readout AISCs.  In the first amplifier choice, the SiPM overvoltage trim and amplification are done inside the TOPSoC ASIC, greatly reducing component count and board space requirements.  Should this prove to be technically unfeasible, a second amplifier method requiring an additional circuit board, requisite components, and engineering effort is costed.
For the photosensors, the Hamamatsu production line of life-extended ALD MCP-PMT is still operating with an expected output of 10 MCP-PMTs/month. The possible further increase of lifetime can be investigated for example by an optimization of the atomic layer thickness.
The option of MCP-PMT replacecment requires several studies and possibly further SiPM developments.
It's important to find best balance among different SiPM's characteristics:
single device size, single cell dimension, operating temperature.
We need to be able to distinguish single photons also after an irradiation of \SI{10 e 11}{n/cm^2} 
%(Fig.~\ref{fig:NeutronFlux})
but keeping a good photon efficiency, a good time resolution with an acceptable thermal and mechanical stress for the detector.

%\clearpage

%% - Fig 3
%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.75]{figs/Neutron17th.pdf}
%\caption{\it Neutron flux per year expected in the photodetector region of the TOP detector as a function of the azimuthal angle. The estimation was done using the $17^{th}$ Monte Carlo campaign and considered an instantaneous luminosity of $8\times 10^{35}cm^{-2}s^{-1}$$.}
%\label{fig:NeutronFlux}
%\end{center}
%\end{figure}

\subsection{Design Development and Human Resources}

The design of the new electronics is still needed.
The design of the new photosensors for the primary option is available, it is the same of the current PMT modules. 
%\subsection{Human Resources}
It is anticipated that for the photosensor upgrade, Nagoya U., INFN/U. Padova and INFN/U. Torino;  while for the electronics upgrade, Indiana U, U. Hawaii, U. Pittsburgh and Nalu Scientific personnel will be the primary contributors.

\subsection{Cost and Schedule}

%\subsection{Common costs}
%
With either amplifier option it is anticipated that one engineer will be involved in the design of the ASIC Carrier board, at 100\% FTE for year 1 and dropping to 50\% FTE for year 2.  Full-time funding for 1 postdoc and 1 graduate student to assist in assembly, test and documentation is requested, under the oversight of faculty members Nishimura and Varner.  Board fabrication and assembly costs are based upon those realized during earlier production. An increase of 20\% is added to account for inflation. As noted earlier, it is assumed that the development costs for the TOPSoC ASIC will have been provided by SBIR funding of Nalu Scientific activities.  Costs are based upon engineering runs in 130~nm CMOS technology.  A yearly firmware development engineering support is costed during the 2 years of production, and at a reduced level during commissioning.
%
%\subsection{Option 1 Costing}
The estimated costs of the electronics upgrade are described in Table~\ref{iTOP:table1} for two options.
In the first option it is assumed that 80 new Carrier boards will be prepared.  The electro-mechanics and cooling of the photosensors are to be provided off-project (INFN + Nagoya U.).  In the second option  an additional "front" board has been considered. The estimated costs for the replacement of the 220 ALD MCP-PMTs are described in Table~\ref{iTOP:table2} for life-extended ALD MCP-PMT option and Table~\ref{iTOP:table3} for the SiPM option.
%
\begin{table}[hp]
\caption{TOP Readout upgrade Amplifier cost estimate.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
\multicolumn{4}{|c|}{\bf option 1} \\ \hline
 Pre-production & Carrier Engineering \& test & 3.0 FTE  & 255 \\ 
 & Parts procur. \& assembly & cost summary & 113  \\ 
  \hline
 Production & Carrier Engineering \& test & 2.5 FTE  & 185 \\
 & Parts procur. \& assembly & cost summary & 376  \\ 
 \hline 
 Commissioning & Engineering \& installation & 1.5 FTE & 105 \\  
 & TOPSoC ASIC support & Nalu Scientific & 80  \\  \hline 
 {\bf Total option 1} & & & {\bf 1,114 k\$} \\ \hline 
\multicolumn{4}{|c|}{\bf option 2 (additional costs)} \\ \hline
%{\bf Phase} & {\bf Resource} & {\bf Basis of estimate} & {\bf Cost (k\$)} \\ \hline
 Pre-production & Front Engineering & 0.2 FTE engr. & 40 \\ 
 & Parts procur. \& assembly & Engr. est. & 5  \\ \hline
 Production & Front Engineering & 0.15 FTE engr. & 30 \\  
 & Parts procur. \& assembly & Engr. est. & 67 \\ \hline 
 Commissioning & Integration & 0.05 FTE engr. & 10 \\  \hline 
 {\bf Total option 2} & & & {\bf 152 k\$} \\ \hline 
{\bf Total opt. 1+2} & & & {\bf 1,266 k\$} \\ \hline \hline
\end{tabular}
\label{iTOP:table1}
\end{table}
%\subsection{TOP Readout Upgrade Cost Summary}
%Depending upon the amplifier option chosen, the total cost will be roughly $1.1-1.3$ M\$.  
%\subsection{MCP-PMT option upgrade costing}
\begin{table}[ht]
\caption{Life-extended ALD MCP-PMT upgrade cost est.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Production & MCP-PMT Production & Engr. est. & 1500 \\  
           & MCP-PMT Test & Engr. est. & 15 \\
           & Assembly parts & Engr. est. & 50  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
{\bf Total} & & & {\bf 1615 k\$} \\ \hline \hline
\end{tabular}
\label{iTOP:table2}
\end{table}
%
\begin{table}[ht]
\caption{SiPM upgrade cost est.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Pre-production & Engineering & 0.5 FTE & 50\\ 
 & SiPM R\&D & Engr. est. &  10 \\ 
 & Cooling R\&D & Engr. est. & 30 \\ \hline
 Production & Engineering & 0.5 FTE & 50 \\  
 & SiPM + assembly parts & Engr. est. & 700 \\
 & Cooling system & Engr. est. & 50  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
 {\bf Total} & & & {\bf 930 k\$} \\ \hline \hline
\end{tabular}
\label{iTOP:table3}
\end{table}



==> 06.OuterDetector/S1.TOP_RFSoC.tex <==
\section{TOP}
\label{sec:TOP}
\editor{E.Torassa}

\subsection{Introduction}

With four years of running experience at Belle II, the world-record luminosity of SuperKEKB has been accompanied by higher than anticipated backgrounds.  For the TOP subsystem this means it is looking increasingly likely that even the life-extended Atomic Layer Deposition Micro-Channel Plate Photomultiplier Tubes (ALD MCP-PMTs) may not survive until the target integrated luminosity.  R\&D has started on a possible silicon photomultiplier (SiPM) replacement option. This option looks promising, although the required cooling will reduce the space available for the readout electronics and limit its acceptable heat load. Anyway thermal gradients and potential thermal and mechanical stresses need to be carefully evaluated. The readout electronics upgrade has been considered as well for different reasons. The projected high rates of Single Event Upsets (SEUs) is problematic, as some number of them are not recoverable and will lead to increasing data taking loss. A more compact electronic 
is expected to reduce SEUs problems, reduce space occupancy and power consumption or in alternative allow to increase the number of channels. This can be achieved by replacing the current 16 IRSX ASICs and 4 Xilinx FPGAs used in the 4 "Carrier" cards of every "board stack" with only one or four new generation RFSoCs performing at the same time analog signal sampling and data aggregation. 
The possibility to have more space and readout more channels is relevant in particular for the SiPM option. 
Perhaps of greater concern is the known/measured lack of radiation tolerance of the fiber optic transceiver modules. 
The timescale for replacement of the TOP photosensors is related to the level of background during the next years. Fig.~\ref{fig:QEprojection} shows the expected projection of PMT quantum-efficiency (QE) degradation. The Monte Carlo expected background was considered for the components related to the luminosity (Bhabha scattering, two-photon processes) and a maximum limit of 5 MHz/PMT for the other components (beam-gas, Touschek). In this case, the QE of normal ALD type PMTs will become less than 80~\% starting from 2027 and all PMTs will reach this level of QE degradation at around the end of the current luminosity target.

Planning has started for these upgrades happening during a possible long shutdown to rebuild the interaction region on the timescale of roughly 5 years from now. 

%Fig. 1
\begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.5]{figures/TOP/TOP-PMT-QE.pdf}
\caption{\it Expected projection of QE degradation for the three different generations of MCP-PMTs installed in the TOP detector: conventional, ALD and life-extended ALD.  Horizontal axis shows the year and vertical axis is the relative QE.}
\label{fig:QEprojection}
\end{center}
\end{figure}

\subsection{Executive Summary}

The rudimentary schedule and cost estimates for the electronic readout are based upon production and delivery of the 8k channels of TOP readout.  This endeavor leverages heavily two sizeable past and new investments: re-use of existing infrastructure and firmware, wherever possible.
In both cases the pre-production plus production timescale is approximately 2 years, with 6-9 months for installation and commissioning.  Based upon the preliminary prototyping being performed and costed separately from this, the total project cost is estimated to be 3.6-6.1 M$\$$ for upgrades to the TOP readout systems.

For the photosensors the primary option is the replacement of normal ALD PMTs with life extended ALD MCP-PMTs once the installed PMTs approach the end of their lifetime.
With this option, we need ~220 new MCP-PMTs to replace normal ALD type PMTs, which costs is estimated to be 1.5 M$\$$. The production of life-extended ALD MCP-PMT already restarted, 90 MCP-PMTs have been ordered, 30 of them have been delivered. A further improvement in the ALD technology
and the MCP-PMTs replacement with cold SiPMs are the possible solutions if the increase of luminosity leads to a rapid loss of efficiency of the life extended ALD MCP-PMTs.

%\clearpage

\subsection{Upgrade Proposal}

The goals of baseline upgrade to the readout electronics are twofold: reduce significantly their size, as well as the power required.  Both goals facilitate the implementation of the requisite cooling needed to operate the SiPMs in single-photon detection (though with significantly increased dark-count) mode.

In order to reduce cost and development time, much of the existing software, firmware and hardware infrastructure can be retained.  The boundary conditions considered for this costing exercise are:

\begin{itemize}
    \item Retain the Standard Control Read-Out Data (SCROD) board, the existing cables and low-voltage power system
    \item Remove the HV divider chain/delivery board and associated cables
    \item Employ a new digitizer solution, each with multiple Gbps connections to the SCROD FPGA
    \item 2 different digitizer options are considered and costed (AMD/Xilinx RF System on Chip and custom TDC ASIC)
\end{itemize}

%The basic revised architecture is illustrated in Fig.~\ref{fig:TOPupgrade}, where the interface plane to the PMTs is pushed back from the current PoGO pin location and is serviced by a single, new Carrier card containing four 32-channel TOPSoC ASICs, which communicate directly with the retained SCROD Rev B.

%\begin{figure}[h]
%\begin{center}
%\includegraphics[scale=0.75]{figs/TOPupgrade.pdf}
%\caption{\it Baseline design for upgrade of the readout "boardstack". A photo at left, and at right schematically
%the proposed replacement.}
%\label{fig:TOPupgrade}
%\end{center}
%\end{figure}
 
Based upon this proposed modification, the upgraded readout system still consists of 64 "board stacks" and still consists of 4 "Carrier" cards per "board stack". First digitizer option being considered is to replace the four 8-channel readout ASICs per carrier card with a single Radio Frequency System on Chip (RFSoC) from AMD/Xilinx as a baseline option. Additional studies are being done to determine if all 128-channels of a board stack can be frequency domain multiplexed into a single RFSoC for potential cost savings. Second digitizer option is to implement a custom Time-to-Digital (TDC) ASIC per carrier card that is able to accept very short pulses ($\sim$400 ps wide) from commercial high speed comparators that asset on the raw, unshaped photon detector signals. This option is under consideration due to the remarkable advancements in commercial high-speed comparators over the past decade and as a less expensive option to the baseline RFSoC option. 
% In the first amplifier choice, the SiPM overvoltage trim and amplification are done inside the TOPSoC ASIC, greatly reducing component count and board space requirements.  Should this prove to be technically unfeasible, a second amplifier method requiring an additional circuit board, requisite components, and engineering effort is costed.

For the photosensors, the Hamamatsu production line of life-extended ALD MCP-PMT is still operating with an expected output of 10 MCP-PMTs/month. The possible further increase of lifetime can be investigated for example by an optimization of the atomic layer thickness.
The option of MCP-PMT replacement requires several studies and possibly further SiPM developments.
It's important to find best balance among different SiPM's characteristics:
single device size, single cell dimension, operating temperature.
Considering the expected neutron rate near the photodetector region at an instantaneous luminosity of $8\times 10^{35}cm^{-2}s^{-1}$  is about \SI{2.5 e 10}{n/(cm^2 \cdot~years)} (Fig.~\ref{fig:NeutronFlux}), we need to be able to distinguish single photons at least up to an irradiation of  \SI{1 e 11}{n/cm^2}, even more for higher luminosity. We need also to keep a good photon efficiency, a good time resolution and have acceptable thermal and mechanical stresses for the detector.

%\clearpage


\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.75]{figures/TOP/Neutron19th.pdf}
\caption{\it Neutron flux per year expected in the photodetector region of the TOP detector as a function of the module number. The estimation was done using the $19^{th}$ Monte Carlo campaign and considered an instantaneous luminosity of $8\times 10^{35}cm^{-2}s^{-1}$.}
\label{fig:NeutronFlux}
\end{center}
\end{figure}

The single channel active area of the MCP-PMT with 16 channels and $1~in^2$ size is about $6 \times 6~cm^2$ anyway smaller SiPMs have been considered to limit the impact of the dark count rate to the single photoelectron spectrum. This will require an increase in the number of channels or a multiplexing downstream of the SiPM amplification.
Sixteen Hamamtsu SiPMs  $1.3 \times 1.3~cm^2$ size and 50 $\mu m$ cells have been irradiated from \SI{1.03 e 09}{n/cm^2} to \SI{5.07 e 11}{n/cm^2}. The single photon spectra are shown in Fig.~\ref{fig:SinglePhoton} for two different irradiation at different temperatures.
In the most critical condition with \SI{5.07 e 11}{n/cm^2} and 20\textdegree C the single photon peak cannot be distinguished from the dark count background.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.60]{figures/TOP/SinglePhotonSpectrum.pdf}
\caption{\it Single photoelectron spectrum for an irradiation of \SI{5.07 e 11}{n/cm^2} (left) and  \SI{5.07 e 10}{n/cm^2} (right) at different temperatures.}
\label{fig:SinglePhoton}
\end{center}
\end{figure}

\subsection{Design Development and Human Resources}

The design of the new electronics is still needed.
The design of the new photosensors for the primary option is available, it is the same of the current PMT modules. 
%\subsection{Human Resources}
It is anticipated that for the photosensor upgrade, Nagoya U., INFN/U. Padova and INFN/U. Torino;  while for the electronics upgrade, Indiana U, U. Hawaii, U. Pittsburgh and SLAC National Accelerator Laboratory personnel will be the primary contributors.

\subsection{Cost and Schedule}

%\subsection{Common costs}
%
It is anticipated that one engineer will be involved in the design of the carrier card board, at 100\% FTE for year 1 and dropping to 50\% FTE for year 2.  Full-time funding for 1 postdoc and 1 graduate student to assist in assembly, test and documentation is requested, under the oversight of U. Hawaii instrumentation frontier professor. Board fabrication and assembly costs are based upon those realized during earlier prototyping. A yearly firmware development engineering support is costed during the 2 years of production, and at a reduced level during commissioning. 

The estimated costs of the electronics upgrade are described in Table~\ref{iTOP:table1} for two digitizer options. The estimated costs for the replacement of the 220 ALD MCP-PMTs are described in Table~\ref{iTOP:table2} for life-extended ALD MCP-PMT option and Table~\ref{iTOP:table3} for the SiPM option.

%
\begin{table}[hp]
\caption{TOP readout electronics upgrade estimate.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{4}{|c|}{\bf Option1: 32-Channel RFSoC Baseline} \\ \hline
{\bf Phase}    & {\bf Resource}              & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
Pre-production & Engineering \& test         & 2.0 FTE       & 1150  \\ 
               & Parts procur. \& assembly   & cost summary  & 100   \\ \hline
Production     & Engineering \& test         & 1.5 FTE       & 890   \\ 
               & Parts procur. \& assembly   & cost summary  & 2,560 \\ \hline
Commissioning  & Integration \& Installation & 0.5 FTE       & 380   \\ \hline
Subtotal       &     \multicolumn{2}{|c|}{}                  & 5,074 \\ \hline
Contingency (20\%) & \multicolumn{2}{|c|}{}                  & 1,015 \\ \hline
Option1 Total Cost & \multicolumn{2}{|c|}{}                  & 6,089 \\ \hline \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{4}{|c|}{\bf Option2: custom TDC ASIC Solution} \\ \hline
{\bf Phase}    & {\bf Resource}              & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
Pre-production & Engineering \& test         & 2.0 FTE       & 1150  \\ 
               & Parts procur. \& assembly   & cost summary  & 100   \\ \hline
Production     & Engineering \& test         & 1.5 FTE       & 890   \\ 
               & Parts procur. \& assembly   & cost summary  & 480   \\ \hline
Commissioning  & Integration \& Installation & 0.5 FTE       & 380   \\ \hline
Subtotal       &     \multicolumn{2}{|c|}{}                  & 3,000 \\ \hline
Contingency (20\%) & \multicolumn{2}{|c|}{}                  & 600   \\ \hline
Option1 Total Cost & \multicolumn{2}{|c|}{}                  & 3,600 \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
\label{iTOP:table1}
\end{table}
%\subsection{TOP Readout Upgrade Cost Summary}
%Depending upon the amplifier option chosen, the total cost will be roughly $1.1-1.3$ M\$.  
%\subsection{MCP-PMT option upgrade costing}
\begin{table}[ht]
\caption{Life-extended ALD MCP-PMT upgrade cost est.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Production & MCP-PMT Production & Engr. est. & 1500 \\  
           & MCP-PMT Test & Engr. est. & 15 \\
           & Assembly parts & Engr. est. & 50  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
{\bf Total} & & & {\bf 1615 k\$} \\ \hline \hline
\end{tabular}
\label{iTOP:table2}
\end{table}
%
\begin{table}[ht]
\caption{SiPM upgrade cost est.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
{\bf Phase} & {\bf Resource} & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
 Pre-production & Engineering & 0.5 FTE & 50\\ 
 & SiPM R\&D & Engr. est. &  10 \\ 
 & Cooling R\&D & Engr. est. & 30 \\ \hline
 Production & Engineering & 0.5 FTE & 50 \\  
 & SiPM + assembly parts & Engr. est. & 700 \\
 & Cooling system & Engr. est. & 50  \\  \hline 
 Commissioning & Integration & 0.5 FTE & 50 \\  \hline 
 {\bf Total} & & & {\bf 930 k\$} \\ \hline \hline
\end{tabular}
\label{iTOP:table3}
\end{table}



==> 06.OuterDetector/S2.KLM-old.tex <==
%%%%%%%%%%%%%%%%%%%%
\section{KLM}
\label{sec:KLM}
\editor{L.Piilonen, X.Wang, G.Varner}

A performance upgrade has been proposed for the Belle II KLM subdetector, which identifies $K_L$ mesons and muons with momenta up to about 4.5 GeV/$c$, to add the capability of energy measurement for the $K_L$ mesons via a time-of-flight measurement. This is described in Sec.~\ref{timing-upgrade}.

An independent upgrade has been proposed to refactor the existing scintillator readout by moving the analog and 
analog-to-digital elements of the readout into the detector panels, simplifying immensely the external connections. This 
upgrade would rebuild each detector panel and replace all existing resistive plate counters (RPCs) with scintillators. 
This is described in Sec.~\ref{readout-upgrade}.

\subsection{KLM geometry and instrumentation}

The KLM subdetector occupies the volume outside the superconducting solenoid, spanning radii of 200--$340~\si{\centi\metre}$ in the 
octagonal barrel and 130--$340~\si{\centi\metre}$ in the forward and backward endcaps. Large-surface-area detector panels of about 
3.1-$\si{\centi\metre}$ thickness are sandwiched in the gaps between the steel plates of the solenoid's magnetic-field flux return. 
Each panel contains either RPCs (barrel layers 3--15) or scintillator strips (barrel layers 1--2, forward-endcap layers 
1--14 and backward-endcap layers 1--12). The RPC cathode readout strips are about $4~\si{\centi\metre}$ wide and each scintillator 
strip is $4~\si{\centi\metre}$ wide, measured orthogonal to a line from the SuperKEKB $e^+ e^-$ collider's interaction point (IP); 
this matches the Moli\`ere radius of muons originating at the interaction point and traversing the electromagnetic 
calorimeter located just inside the solenoid. Each detector panel provides two orthogonal measurements of a 
through-going particle's position via hits on these strips.  There are about 38,000 readout channels in the KLM, of 
which half are for the scintillators.

The cross section of each barrel scintillator strip is $4~\si{\centi\metre} \times 1~\si{\centi\metre}$, so each panel in layers 1--2 
contains 54 $z$-readout strips and between 38 and 69 $\phi$-readout strips, for a total of 93 to 124 strips. The cross section of 
each endcap scintillator strip is $4~\si{\centi\metre} \times 0.75~\si{\centi\metre}$; each panel contains 75 $x$-readout strips and 75 
$y$-readout strips for a total of 150 strips. Photons from each scintillator strip are collected by an embedded wavelength-shifting 
optical fiber (Kuraray Y11(200)MSJ) and detected by a Silicon Photomultiplier (SiPM), also known as a Multi-Pixel Photon 
Counter (MPPC: Hamamatsu S10362-13-050C)---an avalanche photodiode operated in Geiger mode. This solid-state device is 
affixed directly to the scintillator strip at one end of the WLS fiber.  The fiber's other end is mirrored. The signals 
(preamplified internally by a factor of $\sim$10 for the scintillators) are routed via ribbon cables to external readout 
electronics mounted on the magnet yoke.

\subsection{Timing upgrade for $K_L$ momentum measurement}
\label{timing-upgrade}

There is no marked difference in the current particle-identification performance measures between RPCs and 
scintillators. However, the scintillator readout can be upgraded to provide a precise time-of-flight measurement for 
the hit clusters that arise from hadronic interactions of a $K_L$ meson in either the yoke steel or in the ECL (with 
shower leakage into the KLM). This measurement can be converted into determining the $K_L$ meson's energy, 
which is not measurable in the present KLM. Also, the precise hit-time measurement can be applied to a neutron's primary 
hit in a single one-dimensional scintillator strip to better reject out-of-time neutron backgrounds that would 
otherwise contaminate the prompt $K_L$-candidate population.

As in a typical time-of-flight (TOF) counter based on scintillators, it is possible to achieve a precise time 
measurement of a hadronic cluster created by a neutral hadron, such as $K_L$ or a neutron. Converting this to an energy 
measurement and then combining it with the present direction measurement (assuming that the hadronic cluster originated 
from the IP), the four-momentum of a neutral hadron can be determined.
% 
% The momentum magnitude $p$ of a neutral hadron of mass $m$ is related to its time of flight $t$ from the IP via
% \begin{equation}
%     p = \gamma mv = \frac{mcL}{\sqrt{t^2c^2 - L^2}}
% \end{equation}
% where $L$ is the flight distance between the hadronic cluster and the IP. Therefore, the uncertainties $\delta t$ and 
% $\delta p$ are related via
% \begin{equation}\label{eq:tofklm}
%     \frac{\delta t}{\delta p} = - \frac{m^2 L^2}{t\cdot p^3} = - \frac{m^2 L v}{p^3}.
% \end{equation}
% Assuming typical values of $L = 2~\si{\metre}$, $\gamma =3$ and $p \approx 1.5~\hbox{GeV}/c$ of a $K_L$ meson, a
A time resolution of $\delta t = 100~\si{\pico\second}$ {\color{blue} and a flight length of $2~\si{\meter}$} translate into a momentum 
resolution of $\delta p = 0.19~\hbox{GeV}/c$ {\color{blue} for a $K_L$ with a momentum of $1.5~\hbox{GeV}/c$} or a fractional momentum 
resolution of $\delta p/p \approx 13\%$. 

To measure the $t$ of a neutral hadron precisely, both the start and stop times have to be measured.
% The start time is 
% taken from the $e^+ e^-$ collision time provided by SuperKEKB with a resolution % of about $30~\si{\pico\second}$. The lifetime of a $B$ 
% meson or a $D$ meson produced at the IP is about 1--$10~\si{\pico\second}$. 
% Therefore, the start-time resolution is less than $32~\si{\pico\second}$.
The start-time resolution is less than $32~\si{\pico\second}$, dominated by the $e^+ e^-$ collision-time determination. The stop time will be 
measured to a comparable precision from the collection of hits in the hadronic cluster in the new KLM.
% A preliminary study using a KLM-like geometry with a flight distance between the % IP and the detector of 
% $L = 2~\si{\metre}$ was performed using Geant4, which shows a spatial resolution % for the cluster centroid better than $5~\si{\centi\metre}$. 

% R\&D studies in the lab were performed with a setup similar to that of the current KLM scintillators. The same fibers 
% and preamplifiers but new photosensors and scintillator strips are used.
% The photosensor is MPPC type S13360, which has 
% a low dark count rate and operates at about $55~\si{\volt}$. 
% The new scintillator strips are covered by Teflon. The time 
% resolution of the existing preamplifier is found to be about $400~\si{\pico\second}$, which is too coarse for a precise time 
% measurement. Overall, the time resolution of such a detector channel of scintillator+fiber+MPPC and preamplifier is 
% about $1.0-1.5~\si{\nano\second}$. This may be due to the low light collection by the WLS fiber as well as resolution-degrading effects 
% of light absorption and re-emission in the WLS fiber. 
% 
With several years of R\&D in hand, it is found that the combination of a scintillator with long attenuation length
\textit{and without an embedded wavelength-shifting fiber}, large-area photosensor, and a new preamplifier with improved timing can 
achieve the desired time resolution. Photosensors with $6\times 6~\si{\milli\metre}^2$ area from Hamamatsu and NDL (Beijing) are tested. 
{\color{blue} The R\&D includes designing a new preamplifier for SiPM, studying the performance of different SiPMs and how to combine the 
SiPMs in an array, the time resolution of a detector channel with a long length, Geant4 simulation, and algorithm of fetching the stop 
time of $K_L$ from a hadronic cluster and physics performance with the momentum of a $K_L$ could be measured.}
%Figure~\ref{fig:new_SiPM_readout} shows testing with the new Hamamatsu MPPC (S14610-6050HS, powered at $V_{\rm BR} \approx 38~\si{\volt}$) 
%and a newly designed preamplifier. With a laser whose time resolution is $100~\si{\pico\second}$, clearly distinguished peaks of $n$ 
%photoelectrons ($n = 1,\ 2,$ ...) are seen in Fig.~\ref{fig:new_SiPM_readout} (right). This setup shows a time resolution of 
%$45\pm 1~\si{\pico\second}$. Another test with the NDL photosensor (EQR15 11-6060D-S, powered at $V_{\rm BR} = 28.0\pm 0.2~\si{\volt}$) 
%shows a time %resolution of $32.9\pm 0.4~\si{\pico\second}$. 

%\begin{figure}[htb]
%\begin{center}
%%\includegraphics[scale=0.5]{fig/KLM/TOP-PMT-QE.pdf}
%\includegraphics[width=0.35\textwidth]{fig/KLM/SiPM_new_laser.png}
%\includegraphics[width=0.55\textwidth]{fig/KLM/SiPM_new_pe.png}
%\caption{\sl Left: two sets of new photosensors with newly designed preamplifier and a laser source. Right: the ADC 
%distribution shows clear peaks of p.e.}
%\label{fig:new_SiPM_readout}
%\end{center}
%\end{figure}

\subsubsection{Preamplifer for SiPM}

{\color{blue} The new Hamamatsu MPPC (S14610-6050HS, powered at $V_{\rm BR} \approx 38~\si{\volt}$) and  the NDL photosensor 
(EQR15 11-6060D-S, powered at $V_{\rm BR} = 28.0\pm 0.2~\si{\volt}$) are tested and supposed to have good time resolutions. 

To achieve a good time resolution from SiPM, a compact preamplifier with high-speed and low-noise is designed~\cite{pream_sipm}. The 
preamplifier has a good gain stability, a bandwidth of 426 MHz, a baseline noise of $\sigma \approx 0.6 \si{\milli\volt}$, a dynamic 
range up to $170~\si{\milli\volt}$ of the amplitude of the input signal. The setup for studying the time resolution can be achieved 
by combining the preamplifier and different SiPMs, as shown in Fig.~\ref{reso_comb}. A good time resolution of about 
$20~\si{\pico\second}$ is achieved with various SiPMs. Meanwhile, pole-zero cancellation (PZC) is used in the preamplifier to reduce 
the long tail falling time of a SiPM pulse. In the setup shown in Fig.~\ref{reso_comb}, the falling time is reduced to about 
$5~\si{\nano\second}$, and there is no pile-up even when the laser works at a frequency of 20 MHz.} 

\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/diagram_time_reso_SiPM_pream.png}\\
\includegraphics[height=4.0cm]{fig/KLM/Setup_SiPM_pream.jpg}
\includegraphics[height=4.0cm]{fig/KLM/Tsipm_reso_Nphoton.jpg}
\caption{The measurement of the time resolution of preamplifier and SiPM in photon detection. The top shows the 
diagram of the setup for the measurement, and (a) at the bottom shows the picture of the setup containing the laser, 
the SiPMs and the preamplifiers in a dark box. Plot (b) at the bottom shows the measured time resolution versus the 
number of detected photons using various SiPMs.}
\label{reso_comb}
\end{figure}

\subsubsection{Time resolution of a long scintillator bar}

{\color{blue} $K_L$ is detected from the hadronic cluster in KLM. To measure the time of flight of $K_L$,  
several inner layers of the KLM should use detector modules with good time resolution, such as a scintillator with 
a long attenuation length. Several samples are tested, including the BC420 for reference and scintillator strips from 
GaoNengKeDi company in Beijing. Some GaoNengKeDi scintillator strips with a length of $1~\si{\meter}$ have shown 
excellent performance. Figure~\ref{fig:klmtof} shows the test with two strips of a geometry of $2~\si{\centi\meter} 
\times 5~\si{\centi\meter}\times 1~\si{\meter}$ and arrays of 12 SiPMs as the photosensors at two ends of one strip. The 
12 SiPMs are mounted in parallel or series on a PCB. Two short strips with a length of $10~\si{\centi\meter}$ are laid in 
the middle of the long strips to trigger the cosmic rays. The ADC distributions from the cosmic ray tests show a high  
efficiency close to 100\%. SiPMs in series show a better time resolution, which is about $70~\si{\pico\second}$, but a bit 
smaller pulse height of signal. Test with SiPMs in hybrid shows a good balance between time resolution and pulse height.}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/ToF_testing.png}
\caption{Test on $1~\si{\meter}$ long scintillator bar from GaoNengKeDi with cosmic rays. The left on top shows the 
picture of the setup, which has two compact SiPM arrays on the PCB for readout. The right on top shows the signal pulse 
displayed on the Tektronix MDO3024 oscilloscope. The two distributions with fitted curves on the left bottom show the time 
resolutions from the test, in which a time resolution of $70~\si{\pico\second}$ is achieved. The scattering plots of the ADCs 
show large signals with good photon collection and high efficiency. }
\label{fig:klmtof}
\end{figure}

{\color{blue}
To maintain the required timing precision, a robust time-calibration protocol with frequent updates several times per 
day will be necessary for the TOF-like KLM. A cosmic ray test with six strips, which have about $130~\si{\pico\second}$ in 
each strip, and a time calibration with laser divided and fed in the six channels, yield a distribution of $3.1 \pm 
0.4~\hbox{GeV}/c$ of the cosmic ray momenta. This indicates that signal from a laser is a good option for time 
calibration. }

\subsubsection{Geant4 simulation for the $K_L$ momentum determination}

{\color{blue}
A new KLM with 16 super layers of scintillator modules for the time of flight determination is simulated with Geant4, 
as shown in Fig.~\ref{G4_simulations}. The simulation uses the structure of KLM, a scintillator with a long attenuation 
length, SiPM arrays at both ends of one scintillator strip, etc. $K_L$ mesons and muon tracks with $1.~\hbox{GeV}/c$ are 
generated in particle gun in Geant4. Figure~\ref{G4_simulations} shows the structure and the hits from a muon track or a 
hadronic cluster of $K_L$. The muon tracks show very clean hits; however, a hadronic cluster of $K_L$ is much 
more complicated, and it is difficult to get the arrival time of $K_L$ in KLM. A sophisticated algorithm is required to determine the 
arrival time of $K_L$ in the hits. A preliminary study to get the fastest hits shows a reasonable time resolution of 
$FWHM \approx 240~\si{\pico\second}$, as shown in Fig.~\ref{G4_simulations}. Fitting to this distribution with a Gaussian 
function yields $\sigma = (95 \pm 4)~\si{\pico\second}$, while the fit quality is not very good.}


\begin{figure}[htbp]
\centering
\includegraphics[height=4.0cm]{fig/KLM/G4_muon_hits.png}
\includegraphics[height=4.0cm]{fig/KLM/G4_KL_hits.png}\\
\includegraphics[height=4.0cm]{fig/KLM/G4_KL_time_layers.png}
\includegraphics[height=4.0cm]{fig/KLM/G4_KL_hit_number.png}
\caption{Geant4 simulation on a new KLM with scintillator module for the time of flight measurement. On the top, the left 
(right) plot shows the hits from a muon track ($K_L$ cluster) with a momentum of $1~\hbox{GeV}/c$}
\label{G4_simulations}
\end{figure}

{\color{blue} A typical hadronic cluster will contain one to $\approx 30$  hits in the KLM, depending on the parent hadron's 
energy. Combining the hit times of the multiple 2D hits in a more energetic hadron-induced cluster can improve the 
time resolution further; such an improvement is needed at the higher $K_L$ or neutron momenta.}

\subsubsection{Physics performance with a new KLM}

%With the new photosensor and preamplifier, a pair of 
%$4~\si{\centi\metre} \times 1~\si{\centi\metre} \times 10~\si{\centi\metre}$
%scintillator strips with new scintillation material having long attenuation 
%length is tested.
% \textit{This strip does not contain a WLS fiber nor any bore for such a fiber.} 
% Figure~\ref{fig:new_SiPM_scint_timereso} shows a setup with two adjacent scintillator strips coupled to the new 
% photosensor and preamplifier. One strip has a geometry of $4~\si{\centi\metre} \times 1~\si{\centi\metre} \times 10~\si{\centi\metre}$, and 4 pieces of 
%Four $6\times 6~\si{\milli\metre}^2$ SiPMs are combined and mounted to one end of each strip. Preliminary testing with cosmic rays 
%illuminating both strips shows a time resolution of $127.8\pm 3.0~\si{\pico\second}$ per strip. There is additional capacity to 
%improve this overall time resolution by using a better ground in the readout electronics, increasing the visible-light 
%yield from the scintillator and/or the collection of light by the photosensor(s) at the end of the strip.
% In the latter 
% case, one might attach more photosensors  at the collection end of the scintillator strip to collect more of the 
% scintillation light produced in the strip. This is feasible, considering the low price of such photosensors.
%Having multiple photosensors at the end of the scintillator strip is feasible, considering their low price.
%The cross-sectional shape of the new scintillator can be re-optimized to improve the light yield per strip while not 
%sacrificing the positional resolution for IP-originating muons. The coupling between the end of the scintillator strip 
%and the photosensor active surface can be improved as well.
% Finally, one might consider instrumenting both ends of a 
% strip with photosensors to double the prompt collected-light signal instead of having delayed light arrive at the 
% photosensor from a mirrored end, since this does not improve the leading-edge timing resolution. The last option is 
% challenging because of the limited geometric access to the presently mirrored end of each strip and the resulting loss 
% of acceptance.
% 
% \begin{figure}[h]
% \centering
% \includegraphics[height=4.0cm]{fig/KLM/scint_strips.jpg}
% \includegraphics[height=4.0cm]{fig/KLM/SiPM_2scint_time_reso.png}
% \caption{\sl Left: cosmic ray testing with two new designed scintillator channels. Right: the time difference
% between the two channels.}
% \label{fig:new_SiPM_scint_timereso}
% \end{figure}

% A typical hadronic cluster will contain a varying number of 2D hits in the KLM, which acts as a sampling hadronic 
% calorimeter. A low-energy hadronic cluster might have only one 2D hit (i.e., two orthogonal scintillator strips), but a 
% more energetic hadron parent will materialize as many more 2D hits, on average. 
%A typical hadronic cluster will contain one to $\approx 20$ 2D hits in the KLM, depending on the parent hadron's energy.
%Combining the hit times of the multiple 
%2D hits in a more energetic hadron-induced cluster can improve the time resolution further; such an improvement is 
%needed at the higher $K_L$ or neutron momenta. A toyMC study shows that ten 2D hits (i.e., twenty strips) with a time 
%resolution of $200~\si{\pico\second}$ for an individual strip yields an average time resolution of less than $50~\si{\pico\second}$.

%To maintain the required timing precision,
%% over the course of the experiment,
%a robust time-calibration protocol with 
%frequent updates several times per day will be necessary for the TOF-like KLM.

\subsection{Scintillator Readout Upgrade}
\label{readout-upgrade}

Leveraging experience from the deployment and operation of the endcap and inner barrel KLM scintillators, there is a 
compelling reason to refactor the readout in a way that eliminates the many kilometers of twisted-pair ribbon 
cables. 
%Figure~\ref{fig3} clearly illustrates the rather baroque and unwieldy system initially developed to support a mandate at the time to use ribbon cable readout.  In addition to being visually unappealing, these ribbon cables are vulnerable to being jostled during the subsequent cabling that went over the top of them.  As a result, a number of groups of 15 channels are inoperable, and currently leave holes in the muon coverage for the 2 innermost scintillators.  
%When considering an upgrade, a much better cabling scheme is dictated.  
%
%\begin{figure}[h]
%\centering
%\includegraphics[scale=0.4]{fig/KLM/baroque.pdf}
%\caption{\sl Overview of the deployed KLM scintillator readout, where the requirement to use ribbon %cables to instrument the detector panels introduced many problems.}
%\label{fig3}
%\end{figure}
%
%Looking at the motherboard, much of the space is empty. 
As an upgrade readout baseline, a more compact readout will be placed inside each detector panel. 
%This eliminates all of the ribbon-cables and the associated RHIC interface 
%card mounted in front of the external motherboard. 
This internal readout interfaces with the external DAQ system via a few optical fibers.

Independently of this proposed readout-electronics upgrade for the newly installed scintillator panels in the barrel 
KLM, progress is underway to address some of the deficiencies of the present readout design for the existing 
scintillator panels in the endcaps and inner two barrel layers. New firmware for the ASICs has been written and tested 
to perform waveform sampling and provide a higher-resolution ($< 1~\si{\nano\second}$) time measurement than is possible with the 
existing latch (binary) readout. This may help determine the energy of slow $K_L$ mesons via time-of-flight 
%(see Eq.~(\ref{eq:tofklm}) in Sec.~\ref{timing-upgrade}) 
but will only be of sufficient precision for momenta below about $0.7\,{\rm GeV}/c$. (This 
waveform sampling can also measure the pulse area, but this measurement is and will remain compromised by the saturation 
of the $\times$10 preamplifiers within the scintillator panels.) At the same time, this waveform sampling 
algorithm will be able to sample the SiPM output just before and after the main pulse and thereby correct for the 
localized shift in the waveform baseline that is expected in the coming years from the accumulated direct dose of 
neutrons in the SiPMs and the resultant increase in the spontaneous single-pixel discharge noise from each SiPM.

Again, independently of this proposal's readout-electronics upgrade, work is underway to improve the algorithm in the 
KLM trigger firmware to more reliably detect and report activity in the KLM arising from track segments (cosmic rays or 
IP-originating), clusters, leakage from the ECL (particularly in the uninstrumented cracks between the ECL barrel and 
endcaps), and the forward polar-angular region outside the CDC coverage. KLM-trigger tracks can then be aligned with 
CDC-trigger tracks in the GRL/GDL. The goal is to be able to trigger on such KLM activity with sufficient purity that 
other conditions, such as a back-to-back requirement on the KLM trigger output, will not be needed. So that the KLM 
trigger can serve as a reliable veto for dark-matter studies.


%\subsection{KLM Readout Development}

Motivated by the considerations described previously, we propose a modified readout design that incorporates the 
following features:
\begin{itemize}
\item Embed the readout ASICs on circuit boards inside new detector panels (including those in the two innermost 
layers); 
\item Develop a compact SCROD (Control and Readout) that resides inside the detector panel;
\item 64-channel HDSoC readout ASICs are employed, each with a high-speed serial connection to the new SCROD FPGA.
\end{itemize}

The main readout card inside the detector panel can accommodate a higher channel density ASIC. The baseline ASIC being considered for 
upgrade of the TARGET ASIC is the HDSoC ASIC, which has four times higher channel density and streaming readout.
%the features of which are illustrated in Fig.~\ref{KLM:fig4}. There are some issues for the HDSoC:
%\begin{itemize}
%\item $4\times$ integration;
%\item Compact power/signal cabling to SCROD;
%\item System on Chip (signal processing),
%\item ``Data push" possible (reduces need for depth since don't wait for L1 trigger);
%\item Possiblility to integrate amplification, SiPM overbias adjustment;
%\end{itemize}

%\begin{figure}[h]
%\centering
%\includegraphics[height=4.0cm]{fig/KLM/HDSoC_1.png}
%\includegraphics[height=3.0cm]{fig/KLM/HDSoC_2.png}
%\caption{\sl Specifications and project status information regarding the 64-channel High-Density %System-on-Chip (HDSoC) 
%ASIC baselined as the readout chip for this costing exercise.}
%\label{KLM:fig4}
%\end{figure}

Employing the HDSoC ASIC, a readout system that integrates into the new barrel scintillator panels 
will consist of 480 ASICs on dedicated cards and 240 SCRODs to service them.
%is illustrated in Fig.~\ref{KLM:fig5}, and lists the number of ASICs and readout cards required.

%\begin{figure}[h]
%\centering
%\includegraphics[height=6.0cm]{fig/KLM/KLM_readoutUp.pdf}
%\caption{\sl Specifications and project status information regarding the 64-channel High-Density %System-on-Chip (HDSoC) 
%ASIC baselined as the readout chip for this costing exercise.}
%\label{KLM:fig5}
%\end{figure}


\subsection{Cost estimation}

%\subsection{Barrel KLM Panels}
\begin{itemize}
\item {\bf Materials Cost Estimate}

Table~\ref{table:materialcost} provides the material-cost estimate for manufacturing new scintillator-strip panels for the outer thirteen 
layers of the barrel KLM as part of the scintillator-readout upgrade described in Sec.~\ref{readout-upgrade}. The material costs are based 
on the actual costs for the same items used to make the scintillator-strip panels for the inner two barrel layers, scaled up by the 
relative sizes and numbers of the panels and inflated at a rate of 3\% per year.
% for the time between when the materials were procured for the inner layers
% vs when they will be procured for the outer layers.
The panel-construction labor cost depends on where the panels are fabricated since some of the personnel might already 
be on the institution's payroll. The low-end estimate is \$1.3M.

% \begin{table}[htb]
% \begin{center}
% \begin{tabular}{lrcrcr}
% \hline
%                 & {\bf L0--1} &                        & {\bf L2--14} & {\bf Inflation} & {\bf Cost} \\
%                 & {\bf Cost} & {\bf Geometry} & {\bf Cost} & {\bf 13 years} & {\bf Estimate} \\
% {\bf Item} & {\bf (2012)} & {\bf scale factor} & {\bf (2012)} & {\bf (1.03/year)} & {\bf (2025)} \\
% \hline
% Scintillator strips & 50,650 & 7.60 & {\it 384,940} & 1.47 & 565,862 \\
% WLS optical fiber & 36,564 & 7.60 & {\it 277,886} & 1.47 & 408,493 \\
% Photosensors & 85,658 & 7.60 & {\it 651,001} & 1.47 & 956,971 \\
% Aluminum, HDPE, etc  & 49,507 & 7.60 & {\it 376,253} & 1.47 & 553,092 \\
% Shipping to KEK & 16,800 & 7.60 & {\it 127,680} & 1.47 & 187,690 \\
% HV modules & 20,672 & 6.67 & {\it 137,816} & 1.47 & 202,590 \\
% HV mainframes & 37,801 & 0.33 & {\it 12,600} & 1.47 & 18,522 \\
% \hline
% Subtotal & & & {\it 1,968,177} & & 2,893,220 \\
% Contingency (20\%) & & & {\it 393,635} & & 578,644 \\
% \hline\hline
% \multicolumn{3}{l}{\bf TOTAL MATERIAL COST} & {\it 2,361,812} & & {\bf 3,471,764} \\
% \hline
% \end{tabular}
% \caption{\sl Materials-procurement cost estimate (US dollars) for the outer thirteen layers of the barrel KLM.}
% \label{table:materialcost}
% \end{center}
% \end{table}
% 
\item {\bf Readout Cost Estimate}

The total cost for the three options is listed in Table~\ref{KLM:table4}. Based upon the preliminary prototyping being performed 
and costed separately from this, the total project cost is estimated to be $\$$3.0M for upgrades to the KLM readout 
system, depending upon amplifier choices.

% \begin{center}
% \begin{table}[h]
% \caption{\sl KLM Upgrade readout Amplifier Option total cost estimates (common + option additional cost).}
% \centering
% \begin{tabular}{ | l | c | c | c | } \hline
% {\bf Amplifier Option} & {\bf Total cost [k\$]} & {\bf Rough Cost [M\$]}  \\ \hline \hline
%  1) HDSoC ASIC internal amplifiers & 1,441 & {\bf 1.4}  \\
%  2) discrete amplifiers & 1,762 & {\bf 1.8}  \\
%  3) dedicated amplifier ASIC & 1,660 & {\bf 1.7}  \\  \hline \hline
% \end{tabular}
% \label{KLM:table4}
% \end{table}
% \end{center}
% 
% \item {\bf Labor Cost Estimate}
% 
% The panel-construction labor cost depends on where the panels are fabricated, since some of the personnel might already 
% be on the institution's payroll. We scale the labor costs incurred at Virginia Tech in fabricating the 
% scintillator-strip panels for the inner two barrel layers to obtain the estimate in Table~\ref{table:laborcost}. The
% labor costs are comprised of the salaries (and fringe benefits) of two new full-time technical staff members and the 
% wages of twelve undergraduates. The salaries of one postdoc and two graduate students were not included.
% 
% \begin{table}[htb]
% \begin{center}
% \begin{tabular}{lrcrcr}
% \hline
%                 & {\bf L0--1} &                        & {\bf L2--14} & {\bf Inflation} & {\bf Cost} \\
%                 & {\bf Cost} & {\bf Geometry} & {\bf Cost} & {\bf 13 years} & {\bf Estimate} \\
% {\bf Item} & {\bf (2012)} & {\bf scale factor} & {\bf (2012)} & {\bf (1.03/year)} & {\bf (2025)} \\
% \hline
% Labor & 178,754 & 5.00 & 893,770& 1.47 & 1,313,842 \\
% \hline\hline
% \multicolumn{3}{l}{\bf TOTAL LABOR COST} & {\it 893,770} & & {\bf 1,313,842} \\
% \hline
% \end{tabular}
% \caption{\sl Labor cost estimate (US dollars) associated with fabricating and testing the scintillator-strip panels for 
% the outer thirteen layers of the barrel KLM.}
% \label{table:laborcost}
% \end{center}
% \end{table}
% 
\item {\bf Cost Estimate for TOF-like KLM}

To achieve a good timing resolution from an upgraded KLM for determining the 4-momentum of a neutral hadron, the innermost layers
% of barrel and endcaps
should be replaced by new scintillators with long attenuation length and large-area photosensors.
% In this case, a rough estimation on additional cost for new scintillators and large-area photosensors are 
% made only, since the cost on labor and readout would be similar.
The cost of scintillators would be about \$1.8M for three innermost barrel layers and about \$0.25M for five innermost endcap layers.
% in the endcaps.If 4 SiPMs per strip are used,
With four SiPMs per strip, the cost for SiPMs will be \$0.3M for the barrel and \$0.17M for the endcaps. Therefore, the additional 
material cost to achieve the timing is about \$2.5M.

\end{itemize}

In summary, the rough estimation on the cost for KLM upgrade is about \$11.4M.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[hp]
\caption{KLM readout electronics upgrade estimate.}
\centering
\begin{tabular}{ | l | l | l | c | } \hline
\multicolumn{4}{|c|}{\bf HDSoC ASIC readout Upgrade } \\ \hline
{\bf Phase}    & {\bf Resource}              & {\bf Basis of est.} & {\bf Cost (k\$)} \\ \hline
Pre-production & Engineering \& test         & 1.5 FTE       & 610  \\ 
               & Parts procur. \& assembly   & cost summary  & 120  \\ \hline
Production     & Engineering \& test         & 1.5 FTE       & 610  \\ 
               & Parts procur. \& assembly   & cost summary  & 733  \\ \hline
Commissioning  & Integration \& Installation & 1.0 FTE       & 445  \\ \hline
Subtotal       &     \multicolumn{2}{|c|}{}                  & 2518 \\ \hline
Contingency (20\%) & \multicolumn{2}{|c|}{}                  & 504  \\ \hline
Option1 Total Cost & \multicolumn{2}{|c|}{}                  & 3022 \\ \hline
\end{tabular}
\label{KLM:table1}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htb]
\begin{center}
\begin{tabular}{lrcrcr}
\hline
                & {\bf L0--1} &                        & {\bf L2--14} & {\bf Inflation} & {\bf Cost} \\
                & {\bf Cost} & {\bf Geometry} & {\bf Cost} & {\bf 13 years} & {\bf Estimate} \\
{\bf Item} & {\bf (2012)} & {\bf scale factor} & {\bf (2012)} & {\bf (1.03/year)} & {\bf (2025)} \\
\hline
Scintillator strips & 50,650 & 7.60 & {\it 384,940} & 1.47 & 565,862 \\
WLS optical fiber & 36,564 & 7.60 & {\it 277,886} & 1.47 & 408,493 \\
Photosensors & 85,658 & 7.60 & {\it 651,001} & 1.47 & 956,971 \\
Aluminum, HDPE, etc  & 49,507 & 7.60 & {\it 376,253} & 1.47 & 553,092 \\
Shipping to KEK & 16,800 & 7.60 & {\it 127,680} & 1.47 & 187,690 \\
HV modules & 20,672 & 6.67 & {\it 137,816} & 1.47 & 202,590 \\
HV mainframes & 37,801 & 0.33 & {\it 12,600} & 1.47 & 18,522 \\
\hline
Subtotal & & & {\it 1,968,177} & & 2,893,220 \\
Contingency (20\%) & & & {\it 393,635} & & 578,644 \\
\hline\hline
\multicolumn{3}{l}{\bf TOTAL MATERIAL COST} & {\it 2,361,812} & & {\bf 3,471,764} \\
\hline
\end{tabular}
\caption{\sl Materials-procurement cost estimate (US dollars) for the outer thirteen layers of the barrel KLM.}
\label{table:materialcost}
\end{center}
\end{table}

\begin{table}[hbt]
\caption{\sl KLM Upgrade readout Amplifier Option total cost estimates (common + option additional cost).}
\centering
\begin{tabular}{ | l | c | c | c | } \hline
{\bf Amplifier Option} & {\bf Total cost [k\$]} & {\bf Rough Cost [M\$]}  \\ \hline \hline
 1) HDSoC ASIC internal amplifiers & 1,441 & {\bf 1.4}  \\
 2) discrete amplifiers & 1,762 & {\bf 1.8}  \\
 3) dedicated amplifier ASIC & 1,660 & {\bf 1.7}  \\  \hline \hline
\end{tabular}
\label{KLM:table4}
\end{table}

\subsection{RPC Avalanche Mode}





\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/RPC_rate_capability.png}
\caption{TBD}
\label{RPC_rate_capability}
\end{figure}


\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/RPC_rate_capability2.png}
\caption{TBD}
\label{RPC_rate_capability1}
\end{figure}




\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/RPC_Efficiency_vs_flux.png}
\caption{TBD}
\label{RPC_Efficiency_vs_flux}
\end{figure}

In this conceptual design, it is crucial to acknowledge the inherent uncertainty in both the expected particle flux at the designed luminosity and the RPC efficiency as a function of particle flux. Particularly challenging is the prediction of the background neutron flux, underscoring the importance of achieving a higher rate capability to ensure sustained high efficiency at the designed luminosity. While replacing the RPCs with scintillators would undoubtedly achieve this goal of higher rate capability, it should be noted that this option is not only financially and temporally demanding but also carries the potential risk of damaging components within the overall detector system. In this section, we explore the feasibility of shifting the readout mode of the existing RPCs from streamer mode to Avalanche mode. We also delve into the necessary modifications concerning the front-end electronics, gas mixture, and operating voltage.

The rate capability, among other factors, is inversely proportional to the average charge produced by an incident particle \cite{prop:ImprovingTheRPCratecapability}. 

$$\text { Rate Capability }=\frac{1}{\rho t<Q>}$$

Where $\rho$ is the bulk resistivity, $t$ is the total thickness of electrodes $<Q>$  is the average charge delivered in the gas for each count. To enhance the rate capability, it is possible to decrease the average charge per incident. However, this approach is constrained by the existing noise levels within the system and the sensitivity of the readout electronics.


The glass RPCs employed for the KLM have undergone thorough examination and analysis throughout the RnD and operational phases of the BELLE detector\cite{prop:glassRPCSF6} \cite{prop:YAMAGA2000109} \cite{prop:2000Abe} \cite{prop:2000KLMdetectorsubsystem} \cite{prop:2002freonlessoperation}. The average charge values for 2 mm glass RPCs operating with different gas mixtures and under various high voltages are depicted in Fig.~\ref{Charge VS HV}. In these papers, it was established that the charge produced in a streamer event is typically on the order of $100 pC$. 

These values are in a similar order of magnitude as those observed by ATLAS for 2 mm Bakelite RPCs operating in streamer mode \cite{prop:ATLASStreamersuppression} ($\approx30\;pC$),  \cite{prop:ATLASwithCO2} $70 - 120\;pC$ and \cite{prop:ATLASwithEfriendlyGas} $50-60 pC$. The variations in mean streamer charges observed in these references result from the exploration of different gas mixtures and high voltages. Nevertheless, streamer events can be distinguished from avalanche events based on their notably higher charge values and distinct timing characteristics.  



In the past two decades, it has become a prevailing practice to operate RPCs in the so-called avalanche mode, where charge generation is quenched during the avalanche phase, preventing progression to the streamer phase. This can be achieved through a combination of introducing an electron-negative gas like SF6 as a quenching gas and reducing the operating voltage. When graphing efficiency and streamer probability against high voltage, a region characterized by high efficiency and low streamer probability can be identified\cite{prop:ATLASStreamersuppression}. 

\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/KLM_Effieciency_streamer_prop_vs_HV.jpg}
\caption{TBD Efficiency curves in solid lines and streamer probability curves in dashed lines for the standard gas mixture and two selected HFO-based gas mixtures with a muon beam and no background radiation \cite{prop:ATLASwithEfriendlyGas}}
\label{KLM_Effieciency_streamer_prop_vs_HV}
\end{figure}



Fig. \ref{KLM_Effieciency_streamer_prop_vs_HV} displays the dependency of efficiency and streamer probability as a function of the applied high voltage. Within the context of the specific reference paper, the primary emphasis was placed on the examination of diverse gas mixtures. Of particular significance is the identification of a confined region characterized by both high efficiency and low streamer probability, enabling the RPCs to be operated effectively in proportional mode.




\subsubsection{Gas Mixture}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/Charge_VS_HV.png}
\caption{TBD}
\label{Charge VS HV}
\end{figure}




Currently, the RPC operates using a gas mixture consisting of 30\% argon, 8\% butane, and 62\% freon, HFC-134a. Various studies have explored alternative gas mixtures with similar glass RPCs, revealing a noteworthy shift toward lower signal charge while maintaining high efficiency. In particular, the introduction of SF6, characterized by its high electron affinity of $1.05 eV$, appeared to play a crucial role in preventing streamer signals. Ref \cite{prop:glassRPCSF6} primarily focuses on glass RPCs that closely resemble those currently employed in the KLM detector. It conducts a comparative analysis of the gas mixture in use versus three alternatives, all of which contain SF6 and exclude HFC-134a. The study reveals that the overall efficiency remains only slightly lower than that of the current mixture, and, notably, it indicates a reduction in the average charge from $80\;pC$ to a range of $25-40\;pC$. The most noticeable distinction between the RPCs examined in the paper and those currently utilized in our setup is that the paper employs single-gap RPCs, while we use double-gap RPCs. Consequently, it is likely that our efficiency would be slightly higher than theirs. Given that this paper is two decades old, it is highly probable that with recent advancements in front-end electronics, the overall performance could be significantly enhanced. 

%With this understanding, it appears likely that the RPCs can be maintained in operation, even under the more demanding conditions anticipated at design luminosity.



\subsubsection{Readout Electronics}


In this proposal, we aim to minimize the need for replacements as much as possible. However, a drawback of this approach is that we must continue working with the existing cable connections. This is particularly critical for the Z-direction strips, as any modifications to these cables would necessitate opening the detector. The readout of the RPC is accomplished using several meters-long flat-ribbon cables\cite{prop:EoiKLM}. Given these restrictions, the placement of potential new low-noise amplifier front-end electronics can only be accommodated behind the flat ribbon cables. As a result, the initial focus of our R\&D will involve measuring the existing electronic noise levels along the signal line after the flat ribbon cable. It's worth noting that the anticipated signal height is expected to be approximately four to five times smaller than that in streamer mode. Following this step, additional investigations are essential to determine the necessary complexity of the analog-to-digital converter (ADC). Three options are under consideration: 1. Utilizing the existing binary ADC. 2. Introducing a new ADC that includes signal height information. 3. Upgrading to an ADC that offers full waveform readout, akin to the Scintillator readout process. 

Anticipated performance suggests that all components downstream of digitization (packaging) are adequately equipped for operation at design luminosity. As a result, the proposed electronics will comprise two primary components: a compact low-noise amplifier board, mountable directly outside the BKLM, and a digitizer board housing the ADC, alongside an FPG that establishes connectivity with the BELLE2 Data stream.










\begin{figure}[htbp]
\centering
\includegraphics[width=0.8\textwidth]{fig/KLM/RPC_Total_charge_HVeff.png}
\caption{TBD}
\label{RPC_Total_charge}
\end{figure}


Fig. \ref{RPC_Total_charge} from the ATLAS collaboration demonstrates the performance of their newly designed SiGe preamplifier \cite{prop:Cardarelli2013}, indicating that it achieves a 95\% efficiency with a signal height as low as 2 pC, significantly improving upon the previous design, which required 9 pC. It's important to note that in this figure, 'total charge' represents the total charge produced by an incident particle. However, the charge received by the front-end electronics is significantly smaller than this total value.


The figure illustrates simulated efficiency as a function of particle flux for various readout configurations. With the new preamplifier design enabling lower RPC voltages, the charge per incident particle has been reduced, resulting in a substantially improved rate capability. The performance of the new readout system has been experimentally validated at the Gamma Irradiation Facility at CERN, and the observed results align closely with the simulation. This validation demonstrated an improvement in rate capability by approximately one order of magnitude. The KLM RPCs exhibit a bulk resistivity approximately three orders of magnitude higher, resulting in a rate capability roughly three orders of magnitude lower compared to ATLAS. Nevertheless, with a similar upgrade approach, there is potential to increase the rate capability to approximately $10 Hz/cm^2$, a level that adequately accommodates the operational requirements at design luminosity, even when considering the earlier uncertainties discussed in this chapter.


\subsubsection{Working plan}



Upgrading the current RPC system of the KLM detector presents a significant challenge, particularly as numerous detector components are immovably situated and cannot be altered, such as the fixed positioning of the readout cables. Consequently, it is essential to comprehend the existing electronic noise within the system. A limited number of spare RPCs are available for diverse studies, including investigations involving various gas mixtures and different pre-amplifiers. Moreover, it is feasible to create a radiation environment with an incident rate of $1 - 10 Hz/cm^2$ within a typical laboratory setting, although dedicated test beam studies may be required for comprehensive assessments.

==> belle2-uwg-sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%

%% Can be updatd with SVD-specific symbols

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\newcommand{\belletwo}{Belle~II}
%
% Note that latex macros cannot contain numbers, only letters !
%
\newcommand{\phaseone}{Phase~1}
\newcommand{\phasetwo}{Phase~2}
\newcommand{\phasethree}{Phase~3}
\newcommand{\COtwo}{CO$_2$}
\newcommand{\vsep}{$\rm{V}_{\rm SEP}$}
\newcommand{\airex}{AIREX\textsuperscript{\textregistered} }
\newcommand{\apv}{APV25}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\qqbar       {\ensuremath{q\bar{q}}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
%\def\num        {\ensuremath{\nu_\mu}\xspace}
%\def\numb       {\ensuremath{\nub_\mu}\xspace}
%\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}
\def\pis   {\ensuremath{\pi_{\rm s}}\xspace}
\def\pips   {\ensuremath{\pi^+_{\rm s}}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\ma    {\ensuremath{{\rm \,m}^2}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\rm m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


%%%%%%%%%%%%%%%
%% definitions by Tayduganov
%%%%%%%%%%%%%%%
\def\M{\mathcal{M}}
\def\A{\mathcal{A}}
\def\Op{\mathcal{O}^{\,\prime}}
\def\OOp{\mathcal{O}^{\,(\prime)}}
\def\Cp{C^{\,\prime}}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}

%%%%% macros used in theory chapters (Theory, WG9...)
\newcommand{\ov}{\overline}
\newcommand{\Lag}{\ensuremath{\mathcal{L}}}
% Quarks and gluons
%
\newcommand{\qq}{\ensuremath{q}\xspace}
\newcommand{\uq}{\ensuremath{u}\xspace}
\newcommand{\dq}{\ensuremath{d}\xspace}
\newcommand{\sq}{\ensuremath{s}\xspace}
\newcommand{\cq}{\ensuremath{c}\xspace}
\newcommand{\bq}{\ensuremath{b}\xspace}
\newcommand{\tq}{\ensuremath{t}\xspace}
% \newcommand{\qbar}{\ensuremath{\bar{q}}\xspace}
\newcommand{\qbarq} {\ensuremath{q\bar{q}}\xspace} 
%
\newcommand{\ubarq}{\ensuremath{\bar{u}}\xspace}
\newcommand{\dbarq}{\ensuremath{\bar{d}}\xspace}
\newcommand{\sbarq}{\ensuremath{\bar{s}}\xspace}
\newcommand{\cbarq}{\ensuremath{\bar{c}}\xspace}
\newcommand{\bbarq}{\ensuremath{\bar{b}}\xspace}
\newcommand{\tbarq}{\ensuremath{\bar{t}}\xspace}
\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
%\newcommand{\gev}{\,\mbox{GeV}}
%\newcommand{\tev}{\,\mbox{TeV}}
%\newcommand{\mev}{\,\mbox{MeV}}
\newcommand{\eq}[1]{Eq.~(\ref{#1})}
\newcommand{\eqsand}[2]{Eqs.~(\ref{#1}) and (\ref{#2})}
\newcommand{\eqsto}[2]{Eqs.~(\ref{#1}--\ref{#2})}
\newcommand{\ds}{\displaystyle}
\newcommand{\PARITY}{\ensuremath{P}\xspace}
\newcommand{\CCC}{\ensuremath{C}\xspace}
\newcommand{\TTT}{\ensuremath{T}\xspace}
\newcommand{\CP}{\ensuremath{CP}\xspace}
\newcommand{\CPT}{\ensuremath{CPT}\xspace}
\newcommand{\Wb}{\ensuremath{W}\xspace}
\newcommand{\Zb}{\ensuremath{Z}\xspace}
\newcommand{\im}{\mathrm{Im}\xspace}
\newcommand{\real}{\mathrm{Re}\xspace}
\newcommand{\Bodbar}{\ensuremath{\overline{B}{}^{0}_{d}}\xspace}
\newcommand{\bbd}{\ensuremath{B^0_d\!-\!\overline{B}{}^0_d}\,}
\newcommand{\bbmd}{\bbd\ mixing\xspace}
\newcommand{\alpS}{\ensuremath{\alpha_{s}}\xspace}
\newcommand{\LambdaQCD}{\ensuremath{\Lambda_{\text{QCD}}}\xspace}
\newcommand{\MW}{\ensuremath{M_{W}}\xspace}
\newcommand{\GF}{\ensuremath{G_{\text{F}}}\xspace}
\newcommand{\Vqd}{\ensuremath{V_{qd}}\xspace}
\newcommand{\Vqs}{\ensuremath{V_{qs}}\xspace}
\newcommand{\Vqb}{\ensuremath{V_{qb}}\xspace}
\newcommand{\Vud}{\ensuremath{V_{ud}}\xspace}
\newcommand{\Vus}{\ensuremath{V_{us}}\xspace}
\newcommand{\Vub}{\ensuremath{V_{ub}}\xspace}
\newcommand{\Vcd}{\ensuremath{V_{cd}}\xspace}
\newcommand{\Vcq}{\ensuremath{V_{cq}}\xspace}
\newcommand{\Vuq}{\ensuremath{V_{uq}}\xspace}
\newcommand{\Vcs}{\ensuremath{V_{cs}}\xspace}
\newcommand{\Vcb}{\ensuremath{V_{cb}}\xspace}
\newcommand{\Vtd}{\ensuremath{V_{td}}\xspace}
\newcommand{\Vts}{\ensuremath{V_{ts}}\xspace}
\newcommand{\Vtb}{\ensuremath{V_{tb}}\xspace}
\newcommand{\Vtq}{\ensuremath{V_{tq}}\xspace}
\newcommand{\ket}[1]{\ensuremath{\big|{#1}\big\rangle}}
\newcommand{\bra}[1]{\ensuremath{\big\langle{#1}\big|}}
\newcommand{\brax}[1]{\ensuremath{\big\langle{#1}}}   % No ``|''
\newcommand{\braket}[2]{\brax{#1}\ket{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%TDCPV  WG3
\def\permille{\ensuremath{{}^\text{o}\mkern-5mu/\mkern-3mu_\text{oo}}}
\renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}

%%%%%
%% WG6

\def\DstpDzPip{$D^{*+}\rightarrow D^0\pi^+$}
\def\DzKPi{$D^0\rightarrow K\pi$}
\def\DzKK{$D^0\rightarrow \Kp\Km$}
\def\sigmat{$\sigma_t$}
\def\babar{BaBar}
\def\deltam{$\Delta m$}
\def\dWS {D^{0}\to\Kp\pim\piz}
\def\dRS {D^{0}\to\Km\pip\piz}
\def\BES {\text{BES{\ }\uppercase\expandafter{\romannumeral3}}}
\def\BTWO {\text{Belle{\ }\uppercase\expandafter{\romannumeral2}}}
\def\disc {\textcolor{red}{$\bigstar$}}
%\def\evid {\textcolor{red}{$\ding{73}$}}
\def\evid {\textcolor{green}{$\bullet$}}
\def\meas {\textcolor{blue}{$\checkmark$}}
%\DeclareMathOperator\RE{Re}
%\DeclareMathOperator\IM{Im}
\def\ccss{\ensuremath{c\overline c s \overline s}\xspace}
\def\outbdt {\ensuremath{\text{Out}_{\text{FBDT}}}\xspace}
\newcommand{\splot}{\hbox{$_s$}{\cal P}lot}


%%%%%%%%%%%%
%% WG8
\newcommand{\bit}[1]{\boldsymbol{\mathcal{#1}}}
\newcommand{\der}{\stackrel{\leftrightarrow}{D}}
\newcommand{\derleft}{\stackrel{\leftarrow}{D}}
\newcommand{\derright}{\stackrel{\rightarrow}{D}}
\newcommand{\sder}{\not\stackrel{\leftrightarrow}{D}}
\newcommand{\sderleft}{\not\stackrel{\leftarrow}{D}}
\newcommand{\sderright}{\not\stackrel{\rightarrow}{D}}
\newcommand{\psibar}{{\bar{\psi}}}
\newcommand{\re}{\hbox{Re}}
\newcommand{\mpid}{m^2_{\pi}}
\newcommand{\mkd}{m^2_K}

%%%%%%%%%%%%%%
%% svd paper SOFTWARE chapter
\newcommand{\nc}[1]{\texttt{#1}}
\newcommand{\ioct}[1]{\texttt{#1}}
\def\basf{\textit{basf2}}
%\newcommand{\snr}{\ensuremath{\mathrm{S}\hspace{-0.1em}\mathrm{N}\hspace{-0.1em}\mathrm{R}}\xspace}
\newcommand{\snr}{\ensuremath{\mathrm{SNR}}\xspace}
\newcommand{\snrST}{\ensuremath{\snr_\mathrm{strip}}\xspace}
\newcommand{\snrZS}{\ensuremath{\snr_\mathrm{ZS}}\xspace}
\newcommand{\snrADJ}{\ensuremath{\snr_\mathrm{adj}}\xspace}
\newcommand{\snrSEED}{\ensuremath{\snr_\mathrm{seed}}\xspace}
\newcommand{\snrCL}{\snr}
%\newcommand{\snrCL}{\ensuremath{\snr_\mathrm{CL}}\xspace}
\def\uP{u/P\xspace}
\def\vN{v/N\xspace}
\def\traw{\ensuremath{t_{\rm raw}}}
\def\thit{\ensuremath{t_{\rm hit}}}
\def\tZ{\ensuremath{t_0}}
\def\eventtz{event $t_0$}
\def\tZsvd{\ensuremath{t_0^{\rm svdRF}}}
% Tsuboyama 


\usepackage{textgreek}

%\newcommand{\mul}{$\times$}
% \newcommand{\mum}{$\rm{\mu}$m}
%\newcommand{\ohm}{$\rm{\Omega}$}
%\newcommand{\PM}{$\pm$}
% \newcommand{\DEG}{$^\circ$}  use \degrees
%\newcommand{\COtwo}{CO$_2$\ }

\newcommand{\mul}{$\times$}
\newcommand{\um}{\textmu m}
\newcommand{\us}{\textmu s}
% \newcommand{\ohm}{\textOmega}
\newcommand{\PM}{$\pm$}
%\newcommand{\DEG}{$^\circ$}
%\newcommand{\etal}{\textit{et al}.}
\newcommand{\SR}{$^{90}$Sr}


==> titlepage.tex <==
%
% title page
%

